Deadlock-free asynchronous message reordering in Rust with multiparty session types

Rust is a modern systems language focused on performance and reliability. Complementing Rust's promise to provide "fearless concurrency", developers frequently exploit asynchronous message passing. Unfortunately, arbitrarily ordering sending and receiving messages to maximise computation-communication overlap (a popular optimisation to message-passing applications) opens up a Pandora's box of further subtle concurrency bugs. To guarantee deadlock-freedom by construction, we present Rumpsteak: a new Rust framework based on multiparty session types. Previous session type implementations in Rust are either built upon synchronous and blocking communication and/or limited to two-party interactions. Crucially, none support the arbitrary ordering of messages for efficiency. Rumpsteak instead targets asynchronous async/await code. Its unique ability is allowing developers to arbitrarily order send/receive messages while preserving deadlock-freedom. For this, Rumpsteak incorporates two recent advanced session type theories: (1) k-multiparty compatibility (kmc), which globally verifies the safety of a set of participants, and (2) asynchronous multiparty session subtyping, which locally verifies optimisations in the context of a single participant. Specifically, we propose a novel algorithm for asynchronous subtyping that is both sound and decidable. We first evaluate the performance and expressiveness of Rumpsteak against three previous Rust implementations. We discover that Rumpsteak is around 1.7--8.6x more efficient and can safely express many more examples by virtue of offering arbitrary message ordering. Secondly, we analyse the complexity of our new algorithm and benchmark it against kmc and a binary session subtyping algorithm. We find they are exponentially slower than Rumpsteak's.

==> Readme <==




## Docker image
If you just want to run the tests, the easiest way is to use the docker image.

```
$ # download the Dockerfile
$ cd /file/containing/Dockerfile
$ docker build -t rumpsteak-tools .
```

Building the image can take several minutes. Once it is done, the test can be
run as follow:

```
$ docker run -ti --rm rumpsteak-tools:latest examples/Running\ examples/run.sh
```

This command runs several example, from nuscr files to rust API files.


## Installing Rust

To run the artifact, you need to have a working nightly install of Rust. The
easiest way to install Rust is via the Rustup script, which is probably
available via your package manager. In case it is not, you can install it using
the following command, and following the instructions on screen:

```
$ curl --proto '=https' --tlsv1.2 -sSf https://sh.rustup.rs | sh
```

To install a specific version of Rust (in particular, Rust nightly in our case),
run 

```
$ rustup toolchain install nightly
```

and then, select `nightly` as the default toolchain:

```
$ rustup default nightly
```

You should now have a working install of Rust nightly.


## Building the project

First, you have to get the source files:

```
$ git clone https://github.com/zakcutner/rumpsteak; cd rumpsteak # TODO anonymous github
```

The project can then be built:

```
$ cargo build
```

## Top-down approach


==> arxiv/Readme <==




## Docker image
If you just want to run the tests, the easiest way is to use the docker image.

```
$ # download the Dockerfile
$ cd /file/containing/Dockerfile
$ docker build -t rumpsteak-tools .
```

Building the image can take several minutes. Once it is done, the test can be
run as follow:

```
$ docker run -ti --rm rumpsteak-tools:latest examples/Running\ examples/run.sh
```

This command runs several example, from nuscr files to rust API files.


## Installing Rust

To run the artifact, you need to have a working nightly install of Rust. The
easiest way to install Rust is via the Rustup script, which is probably
available via your package manager. In case it is not, you can install it using
the following command, and following the instructions on screen:

```
$ curl --proto '=https' --tlsv1.2 -sSf https://sh.rustup.rs | sh
```

To install a specific version of Rust (in particular, Rust nightly in our case),
run 

```
$ rustup toolchain install nightly
```

and then, select `nightly` as the default toolchain:

```
$ rustup default nightly
```

You should now have a working install of Rust nightly.


## Building the project

First, you have to get the source files:

```
$ git clone https://github.com/zakcutner/rumpsteak; cd rumpsteak # TODO anonymous github
```

The project can then be built:

```
$ cargo build
```

## Top-down approach


==> arxiv/acm.tex <==
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
\providecommand\BibTeX{{%
\normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
\setcopyright{acmcopyright}
\copyrightyear{2018}
\acmYear{2018}
\acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
\acmConference[PPoPP '22]{Principles and Practice of Parallel Programming 2022}{February 12--16, 2022}{Seoul, South Korea}
\acmBooktitle{Principles and Practice of Parallel Programming 2022, February 12--16, 2022, Seoul, South Korea}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}

\begin{CCSXML}
	<ccs2012>
	<concept>
	<concept_id>10011007.10011006.10011066</concept_id>
	<concept_desc>Software and its engineering~Development frameworks and environments</concept_desc>
	<concept_significance>500</concept_significance>
	</concept>
	<concept>
	<concept_id>10010520.10010575.10010577</concept_id>
	<concept_desc>Computer systems organization~Reliability</concept_desc>
	<concept_significance>100</concept_significance>
	</concept>
	<concept>
	<concept_id>10011007.10011006.10011041.10011047</concept_id>
	<concept_desc>Software and its engineering~Source code generation</concept_desc>
	<concept_significance>500</concept_significance>
	</concept>
	</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Software and its engineering~Development frameworks and environments}
\ccsdesc[100]{Computer systems organization~Reliability}
\ccsdesc[500]{Software and its engineering~Source code generation}

\keywords{Rust, Asynchronous Message Passing, Message Reordering, Computation-Communication Overlap, Multiparty Session Types}

%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

\makeatletter
\if@ACM@anonymous
    \renewcommand{\rumpsteak}{\textsc{Ranon}\xspace}
    \renewcommand{\repository}{\cite{Ranon}\xspace}
\fi
\makeatother


==> arxiv/artifact/Artifact_short_content.tex <==

\section{Artifact}

\subsection{Content of the artifact\label{content-of-the-artifact}}

The artifact~\cite{Artifact} contains the following files:

\begin{verbatim}
.
|-- Artifact.md
|-- Artifact.pdf
|-- Dockerfile
|-- gen_fig_6.sh
|-- gen_fig_7.sh
`-- getting_started.sh
\end{verbatim}

Note that an internet connection is required to use the artifact.


\subsection{Getting started guide (Docker artifact)\label{getting-started-guide-docker-artifact}}

In this subsection, we will run the benchmarks used to produce \cref{fig:RuntimeBenchmarks,fig:SubtypingBenchmarks}  of the paper in a Docker container. At the end of this section,
you should be have all the plots of those figures.

\begin{quote}
	Note that the benchmark results may not match those in
	\cref{fig:RuntimeBenchmarks,fig:SubtypingBenchmarks} when run in a
	Docker container or a machine with different specification than used in
	the paper. See the subsection on \emph{Claims supported or not by the
	artifact} for more discussion of this.
\end{quote}

To run the getting started guide, we assume you are running a Linux
machine with Docker and Gnuplot installed, as well as standard Unix
tools (\texttt{tail}, \texttt{awk}, \texttt{cut}, etc.).

This \emph{Getting started} subsection is fully automated: extract the
archive and run the \texttt{getting\_started.sh} script. \emph{The
script takes a long time to run all the benchmarks. On the author's
laptop, it took approximately 2 hours and 15 minutes.} When the script
finishes, you should have a few \texttt{*.png} plots which correspond to
the plots shown in \cref{fig:RuntimeBenchmarks,fig:SubtypingBenchmarks}  of the paper.

	\begin{lstlisting}[language=sh]
$ cd /path/to/extracted/artifact/
$ ./getting_started.sh
	\end{lstlisting}

Once run, to clean-up your system, in addition to removing the archive
folder, you should remove the docker image (the following command
assumes you don't have other docker images/containers on your system):

	\begin{lstlisting}[language=sh]
$ docker rmi rumpsteak_tool
$ docker system prune
	\end{lstlisting}


\subsubsection{Output}

The \texttt{getting\_started.sh} generates figures similar to the one used in
the paper\footnote{They are not exactly the same in the sense that they are not
produced by the same tool (Tikz vs. Gnuplot), but the data they use is produced
similarly.}.

We show in~\cref{fig:ex_fig} the figures \texttt{fft.png} and \texttt{ring.png}
that are the equivalent of \cref{fig:RuntimeBenchmarks} (subfigure~FFT) and
\cref{fig:SubtypingBenchmarks} (subfigure~Ring) in the paper.

\begin{figure}
	\begin{subfigure}[b]{.48\linewidth}
		\includegraphics[width=\textwidth]{fig_6_fft}
		\caption{Figure~\texttt{fig\_6\_fft.png} generated by the artifact,
		which corresponds to Example~FFT in
		\cref{fig:RuntimeBenchmarks} in the paper.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{.48\linewidth}
		\includegraphics[width=\textwidth]{fig_7_ring}
		\caption{Figure~\texttt{fig\_7\_ring.png} generated by the artifact,
		which corresponds to Example~Ring in
		\cref{fig:SubtypingBenchmarks} in the paper.}
	\end{subfigure}
	\caption{Two examples of the figures generated. Note that those figure
	are obtain from a different run of the artifact, in a lower-end
	computer, which explains the differences with figures presented in the
	paper.}
	\label{fig:ex_fig}
\end{figure}

\subsubsection{Analysing the raw data\label{analysing-the-raw-data}}

\paragraph{Runtime benchmarks\label{a.-runtime-benchmarks}}

The results used to generate \cref{fig:RuntimeBenchmarks} are generated with
\href{https://crates.io/crates/criterion}{Criterion}. Criterion produces
the tree of files shown in \cref{fig:criterion}. The report can be viewed in a
web brower.

\begin{figure}
	\begin{center}
\begin{verbatim}
.
|-- double_buffering
|   |-- ...
|-- fft
|   |-- ...
|-- report
|   `-- index.html
`-- stream
    |-- ...
\end{verbatim}
\end{center}
	\caption{The files created by the Criterion benchmark (in
	\texttt{results/criterion/}). A detailed report is available by viewing
	\texttt{index.html} in a browser.}
	\label{fig:criterion}
\end{figure}


\paragraph{Subtyping benchmarks\label{b.-subtyping-benchmarks}}

Hyperfine generates a CSV file (located at \texttt{results/data/*/*.csv}) for the results
of each benchmark. For each row, this file contains

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\item
  \texttt{command}: the actual command that was run;
\item
  \texttt{mean}: the mean time to execute the command;
\item
  \texttt{stddev}: the standard deviation of executing the command;
\item
  \texttt{median}: the median time to execute the command;
\item
  \texttt{user}: the mean \emph{user} time to run the command;
\item
  \texttt{system}: the mean \emph{system} time to run the command;
\item
  \texttt{min}: the minimum time to run the command;
\item
  \texttt{max}: the maximum time to run the command; and
\item
  \texttt{parameter\_n}: the value of the parameter used in the command
\end{enumerate}

where all times are given in seconds. Since we do not care about
execution time spent in the kernel (all relevant computation is done in
user space) we take only the timings in the \texttt{user} column. We
provide a script to plot the mean user execution time against the
parameter value for each tool.

\subsection{Claims supported or not by the artifact\label{claims-supported-or-not-by-the-artifact}}


\subsubsection{Claims supported by the artifact\label{claims-supported-by-the-artifact}}

\begin{itemize}
\item
	Results presented in \cref{fig:SubtypingBenchmarks} are fairly stable across different
  machines, even when run in Docker. One should expect to obtain similar
  plots on their machine.
\end{itemize}


\subsubsection{Claims partially supported by the artifact\label{claims-partially-supported-by-the-artifact}}

\begin{itemize}
\item
	Results presented in \cref{fig:RuntimeBenchmarks} are quite dependent on the number of cores
  provided by the machine and on other programs being run on the machine
  simultaneously. The results presented in the paper are run on a
  16-core AMD Opteron 6200 Series at 2.6GHz with hyperthreading and
  128GB of RAM.

  Attempts run on lower-end processors or from within a Docker container
  may not provide similar results (in particular, the \texttt{rustfft}
  implementation is highly optimised for sequential execution and
  outperforms approaches based on message passing on processors with
  fewer cores). Nonetheless, the performance of Rumpsteak vs.~other MPST
  implementations would remain mostly comparable.
\end{itemize}


\subsubsection{Claims not supported by the artifact\label{claims-not-supported-by-the-artifact}}

\begin{itemize}
\item
  NuScr is an external tool not contributed by the authors, and
  therefore not part of the claims of the paper.
\end{itemize}


==> arxiv/preamble.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bussproofs}
\usepackage{caption}
\usepackage[inline]{enumitem}
\usepackage{footnote}
\usepackage{listings}
\usepackage{pdflscape}
\usepackage{pgfplots}
\usepackage{pifont}
\usepackage{stmaryrd}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{xfrac}
\usepackage{xspace}

\usepackage[capitalize]{cleveref}

\usepackage{rust}

%% TODO Remove
\usepackage{todonotes}

\crefname{section}{\textbf{\S}}{\textbf{\S\S}}
\creflabelformat{section}{#2\textbf{#1}#3}

\crefname{subsection}{\textbf{\S}}{\textbf{\S\S}}
\creflabelformat{section}{#2\textbf{#1}#3}

\crefname{subsubsection}{\textbf{\S}}{\textbf{\S\S}}
\creflabelformat{section}{#2\textbf{#1}#3}

\crefname{line}{l.}{ls.}

\makesavenoteenv{tabular}
\makesavenoteenv{table*}

\def\ScoreOverhang{1pt}
\def\defaultHypSeparation{\hskip 5pt}

\definecolor{ruleColor}{rgb}{0.1, 0.3, 0.1}%
\definecolor{codepurple}{rgb}{.58,0,.82}
\definecolor{codegreen}{rgb}{0,.6,0}

\definecolor{primary}{HTML}{6C8EBF}
\definecolor{secondary}{HTML}{D6B656}
\definecolor{tertiary}{HTML}{82B366}
\definecolor{quaternary}{HTML}{666666}
\definecolor{quinary}{HTML}{B85450}
\definecolor{senary}{HTML}{9673A6}

\usetikzlibrary{arrows, arrows, arrows.meta, automata, backgrounds, calc, fit, matrix, positioning, shapes, spy}
\usepgfplotslibrary{groupplots}
\pgfplotsset{compat=1.16,
  /pgfplots/xbar legend/.style={
      /pgfplots/legend image code/.code={\draw[##1,/tikz/.cd,yshift=-.4em] (0cm,0cm) rectangle (0.8em,0.8em);},
    },
  /pgfplots/ybar legend/.style={
      /pgfplots/legend image code/.code={\draw[##1,/tikz/.cd,yshift=-.4em] (0cm,0cm) rectangle (0.8em,0.8em);},
    },
}

\setlist[description]{
  style=unboxed,
  topsep=0pt,
  leftmargin=0cm,
  listparindent=\parindent,wide
}

\lstset{
  commentstyle=\color{codegreen},
  keywordstyle=\color{magenta},
  keywordstyle=[2]\color{codepurple},
  keywordstyle=[3]\color{codepurple},
  keywordstyle=[4]\color{codegreen},
  keywordstyle=[5]\color{codegreen},
  numberstyle=\sffamily\tiny,
  stringstyle=\color{codepurple},
  basicstyle=\ttfamily\footnotesize\linespread{.9}\selectfont,
  breakatwhitespace=false,
  breaklines=true,
  upquote=true,
  numbers=left,
  showspaces=false,
  showstringspaces=false,
  showtabs=false,
  tabsize=2,
  escapechar=@,
  belowcaptionskip=10pt
}

\lstdefinelanguage{Scribble}{
  sensitive,
  morecomment=[l]{//},
  morecomment=[s]{/*}{*/},
  morestring=[b]{"},
  morekeywords={module, type, as, global, protocol, role, rec, choice, at, or, continue, from, to}
}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

\theoremstyle{remark}
\newtheorem*{remark}{Remark}

\newcommand{\code}[1]{\texttt{#1}}

\newcommand{\async}{\code{async}\xspace}
\newcommand{\await}{\code{await}\xspace}

\newcommand{\amr}{\textsc{AMR}\xspace}
\newcommand{\mpst}{\textsc{MPST}\xspace}
\newcommand{\rumpsteak}{\textsc{Rumpsteak}\xspace}
\newcommand{\multicrusty}{\textsc{MultiCrusty}\xspace}
\newcommand{\ferrite}{\textsc{Ferrite}\xspace}
\newcommand{\sesh}{\textsc{Sesh}\xspace}
\newcommand{\rustfft}{\textsc{RustFFT}\xspace}
\newcommand{\kmc}{\(k\)-\textsc{MC}\xspace}
\newcommand{\concur}{\textsc{SoundBinary}\xspace}
\newcommand{\nuscr}{\textsc{\(\nu\)Scr}\xspace}
\newcommand{\repository}{\cite{Rumpsteak}\xspace}

\newcommand{\ppt}[1]{\code{#1}}

\newcommand{\tbool}{\code{bool}}
\newcommand{\tnat}{\code{nat}}
\newcommand{\tint}{\code{int}}
\newcommand{\tunit}{\code{unit}}

\newcommand{\gt}[0]{\mathsf{G}}
\newcommand{\gtmsg}[3]{\ppt{#1} \to \ppt{#2}: \left\{#3\right\}}
\newcommand{\gtmsgs}[2]{\ppt{#1} \to \ppt{#2}: \{}
\newcommand{\gtmsge}{\}}
\newcommand{\gtvar}[1]{\mathbf{#1}}
\newcommand{\gtrec}[1]{\mu\mathbf{#1}.}
\newcommand{\gtend}{\code{end}}
\newcommand{\gtproj}[2]{#1 \upharpoonright \ppt{#2}}

\newcommand{\lt}[0]{\mathsf{T}}
\newcommand{\tout}[1]{\ppt{#1}!}
\newcommand{\tin}[1]{\ppt{#1}?}
\newcommand{\tsel}[1]{\oplus_{#1}}
\newcommand{\tbra}[1]{\&_{#1}}
\newcommand{\tvar}[1]{\mathbf{#1}}
\newcommand{\trec}[2]{\mu\mathbf{#1}.#2}
\newcommand{\tend}{\mathtt{end}}

\newcommand{\efsm}{\mathsf{M}}
\newcommand{\oefsm}{\mathsf{M}'}
\newcommand{\api}{\mathsf{A}}
\newcommand{\proc}{\mathsf{P}}

\newcommand{\refa}[1]{\ensuremath{\mathcal{A}^{(\ppt{#1})}}}
\newcommand{\refb}[1]{\ensuremath{\mathcal{B}^{(\ppt{#1})}}}
\newcommand{\act}[1]{\code{act}(#1)}
\newcommand{\fterms}[1]{\code{terms}(#1)}
\newcommand{\tr}[1]{\mathcal{T}\left(#1\right)}

\newcommand{\nil}{\varnothing}
\newcommand{\pair}[2]{\langle#1\ \lceil\!\!\rfloor \ #2\rangle}
\newcommand{\triple}[3]{\langle#1,#2,#3\rangle}
\newcommand{\map}[1]{\left[#1\right]}

\newcommand{\si}[1]{\llbracket #1 \rrbracket_{\tiny\texttt{si}}}
\newcommand{\so}[1]{\llbracket #1 \rrbracket_{\tiny\texttt{so}}}
\newcommand{\siso}[1]{\llbracket #1 \rrbracket_{\tiny\texttt{siso}}}

\newcommand{\ruleSub}[1]{\rulename{sub-#1}}
\newcommand{\ruleMrg}[1]{\rulename{mrg-#1}}
\newcommand{\ruleP}[1]{\rulename{proj-#1}}
\newcommand{\ruleAlg}[1]{\rulename{#1}}

\newcommand{\veryshortrightarrow}[1][3pt]{\mathrel{%
    \vcenter{\hbox{\rule[-.5\fontdimen8\textfont3]{#1}{\fontdimen8\textfont3}}}%
    \mkern-4mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}
\newcommand{\reduce}{\shortrightarrow}

%\newcommand{\ruleRed}[1]{\rulename{red-#1}}
\newcommand{\ruleRed}[1]{\rulename{\(\veryshortrightarrow\)#1}}
\newcommand{\ruleRedA}{\ruleRed{$\mathcal{A}$}}
\newcommand{\ruleRedB}{\ruleRed{$\mathcal{B}$}}

\newcommand{\ruleRef}[1]{\rulename{ref-#1}}
\newcommand{\ruleRefA}{\ruleRef{$\mathcal{A}$}}
\newcommand{\ruleRefB}{\ruleRef{$\mathcal{B}$}}

\newcommand{\bnfas}{\mathrel{::=}}
\newcommand{\bnfalt}{\mathrel{\mid}}

\newcommand\proto[1]{{\color{primary}{\code{#1}}}}
\newcommand\feat[1]{\textbf{\scriptsize #1}}
\newcommand\oneshot{{\color{secondary}{\code{oneshot}}}\xspace}
\newcommand\reusable{{\color{secondary}{\code{reusable}}}\xspace}

\newcommand{\rulename}[1]{{\color{ruleColor}\textsc{\small [#1]}}}%

\newcommand{\tick}{{\tiny\ding{52}}}
\newcommand{\ftick}{{\color{tertiary}\tiny\ding{52}}}
\newcommand{\htick}{{\color{secondary}\tiny\ding{55}}}
\newcommand{\cross}{{\color{quinary}\tiny\ding{55}}}

\newcommand{\tsize}[1]{|#1|}
\newcommand{\oh}{\mathcal{O}}

\newtoggle{full}
% CHANGE HERE FOR FULL VERSION
\settoggle{full}{true}
\iftoggle{full}
{
  \newcommand{\inApp}[1]{the \cref{#1}}
}{
  \newcommand{\inApp}[1]{the full version~\cite{FullVersion}}
}


==> arxiv/sections/abstract.tex <==
\begin{abstract}
    %	Asynchronous message passing is a widely-used in concurrent applications
    %	thanks to its efficient and intuitive communication model. In particular,
    %	developers can exploit asynchronous message reordering, where send and are
    %	reordered to maximise computation-communication overlap. However, these
    %	kinds of optimisations are often prone to concurrency bugs such as
    %	deadlocks.

    %	\rumpsteak uses \emph{multiparty session types} and targets
    %	\emph{asynchronous} applications using \code{async}/\code{await} code. Its
    %	unique feature is the ability to facilitate \emph{asynchronous message
    %		reordering} while offering \emph{deadlock-freedom}. For this, \rumpsteak
    %	incorporates two recent advanced session type theories:
    %	\begin{enumerate*}[label=\textbf{(\arabic*)}]
    %		\item \emph{$k$-multiparty compatibility} (\kmc), which \emph{globally}
    %		verifies safety properties for a set of participants and
    %		\item \emph{asynchronous multiparty session subtyping}, which
    %		\emph{locally} verifies optimisations in the context of a single
    %		participant. Specifically, we propose a novel algorithm for asynchronous
    %		subtyping that is both sound and decidable.
    %	\end{enumerate*}
    %	Crucially, none of the previous implementations can support the safe message
    %	reordering in a multiparty context.

    %	We first evaluate the performance and expressiveness of \rumpsteak against
    %	previous Rust implementations, using a range of case studies and benchmarks.
    %	We discover that \rumpsteak is around 1.9--14.5x more efficient and can
    %	safely express many more examples by virtue of offering asynchronous message
    %	reordering. Secondly, we analyse the complexity of our new subtyping
    %	algorithm and benchmark it against \kmc and a previous \emph{two-party}
    %	algorithm. We find these existing algorithms are slower than \rumpsteak's.

    Rust is a modern systems language focused on performance and reliability.
    Complementing Rust's promise to provide "fearless concurrency", developers
    frequently exploit asynchronous message passing. Unfortunately, arbitrarily
    ordering sending and receiving messages to maximise computation-communication
    overlap (a popular optimisation to message-passing applications) opens up
    a Pandora's box of further subtle concurrency bugs.

    To guarantee deadlock-freedom by construction, we present \rumpsteak: a new
    Rust framework based on \emph{multiparty session types}. Previous session
    type implementations in Rust are either built upon synchronous and blocking
    communication and/or limited to two-party interactions. Crucially, none
    support the arbitrary ordering of messages for efficiency.

    \rumpsteak instead targets asynchronous \code{async}/\code{await} code. Its
    unique ability is allowing developers to arbitrarily order send/receive
    messages while preserving deadlock-freedom. For this, \rumpsteak
    incorporates two recent advanced session type theories: (1) $k$-multiparty
    compatibility (\kmc), which \emph{globally} verifies the safety of a set of
    participants, and (2) asynchronous multiparty session subtyping, which
    \emph{locally} verifies optimisations in the context of a single
    participant. Specifically, we propose a novel algorithm for asynchronous
    subtyping that is both sound and decidable.

    We first evaluate the performance and expressiveness of \rumpsteak against
    three previous Rust implementations. We discover that \rumpsteak is around
    1.7--8.6x more efficient and can safely express many more examples by virtue
    of offering arbitrary message ordering. Secondly, we analyse the complexity
    of our new algorithm and benchmark it against \kmc and a \emph{binary}
    session subtyping algorithm. We find they are exponentially slower than
    \rumpsteak's.
\end{abstract}


==> arxiv/sections/case_study.tex <==
\section{Case Study: HTTP Cache}
\label{sec:CaseStudy}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle, white, fill=black, thick, inner sep=1.25pt, outer sep=0pt] (char) {\sffamily\tiny\bfseries#1};}\hspace{1pt}}

\begin{figure}
  \centering
  \sffamily\footnotesize
  \setlength{\twemojiDefaultHeight}{14pt}
  \begin{tikzpicture}[-to, thick, node distance=1.4cm and 2.8cm, every path/.style={shorten >=0.1cm, shorten <=0.1cm}]
    \node[align=center] (C) {\twemoji{technologist}\\\textit{Client}};
    \node[align=center] (P) [right=of C] {\twemoji{desktop computer}\\\textit{Proxy}};
    \node[align=center] (O) [right=of P] {\twemoji{earth_africa}\\\textit{Origin}};
    \node[align=center] (D1) [below=of C] {\twemoji{minidisc}\\\textit{Cache}};
    \node[align=center] (D2) [below=of P] {\twemoji{minidisc}\\\textit{Cache}};
    \node[align=center] (D3) [below=of O] {\twemoji{minidisc}\\\textit{Cache}};

    \path (C) edge node[fill=white] {\circled{0} Request} (P);
    \path[above, bend right=20] (P) edge node {\circled{7} Response} (C);

    \path (P) edge node[fill=white] {\circled{5} Request} (O);
    \path[above, bend right=20] (O) edge node {\circled{6} Response} (P);

    \path[sloped, above, bend right=15] (P) edge node {\circled{1} Lock} (D1);
    \path[sloped] (D1) edge node[fill=white] {\circled{2} Locked} (P);

    \path[sloped, below, bend right=10] (P) edge node {\circled{3} Load} (D2);
    \path[sloped, below, bend right=10] (D2) edge node {\circled{4} Entry} (P);

    \path[sloped] (P) edge node[fill=white] {\circled{8} Store/Remove\textsuperscript{$\star$}} (D3);
    \path[sloped, above, bend left=15] (P) edge node {\circled{9} Unlock} (D3);
  \end{tikzpicture}
  \caption{Interactions in the caching case study (optional interactions are marked with $\star$).}
  \label{fig:Caching}
\end{figure}

Caches are important for the performance of web applications. When a
\emph{client} (e.g.\ a browser) makes an HTTP request to an \emph{origin} (i.e.\
a web server), a \emph{proxy} can often fulfil the request by using a previous
response stored in a \emph{cache}. This reduces strain on the origin since fewer
expensive responses have to be sent and can improve latency if the cache is
physically located closer to the client (this is the concept behind content
delivery networks).

Since \emph{static} resources can change frequently, the HTTP protocol contains
several methods for validating that cache entries are not expired---we make use
of \emph{entity tags}~\cite{Fielding2014}. Here, the origin gives each version
of a resource a unique identifier, which is included in the response. The cache
stores this identifier with each entry. When a new request is made for the same
resource, this identifier is sent to the origin to inexpensively confirm that
the response has not expired.

We build a caching protocol using a microservices architecture shown in
\cref{fig:Caching}. Importantly, the client and origin's implementations are
unaware of the existence of the proxy.

\begin{enumerate*}[start=0, label={\hspace{2pt}\protect\circled{\scriptsize\arabic*}}]
  \item The client makes a request to the origin that is intercepted by the
  proxy.
  \item The proxy locks the entry for that request in the cache. This prevents
  simultaneous requests causing the same response to be returned from the origin
  multiple times.
  \item The cache confirms that the resource has been successfully locked.
  \item The proxy loads the previously-stored response (if any) in the cache.
  \item This entry is returned to the proxy.
  \item The client's request is forwarded to the origin, including the entity
  tag if it was in the cache.
  \item The origin responds to the request.
  \item This response if forwarded to the client. If the origin's response
  simply confirmed that the entity tag was still valid, then the proxy sends the
  cached version.
  \item If the cache entry is empty or its previous value had expired, the new
  response is stored. If the response cannot be cached (e.g.\ it contains no
  entity tag), then this step is skipped and any existing cache entry is removed
  as appropriate.
  \item The cache entry is unlocked so that future requests can be made.
\end{enumerate*}

\begin{lstlisting}[language=Scribble, caption={Scribble protocol for the caching case study.}, label={lst:CachingScribble}, float=h]
global protocol Caching(role Client, role Proxy,
    role Cache, role Origin) {
  Request from Client to Proxy;
  Lock from Proxy to Cache;
  Locked from Cache to Proxy;
  Load from Proxy to Cache;
  Entry from Cache to Proxy;
  Request from Proxy to Origin;
  Response from Origin to Proxy;
  Response from Proxy to Client;
  rec Loop {
    choice at Proxy {
      Store from Proxy to Cache;
      continue Loop;
    } or {
      Remove from Proxy to Cache;
      continue Loop;
    } or {
      Unlock from Proxy to Cache;
    }
  }
}
\end{lstlisting}

To demonstrate that \rumpsteak is applicable to larger use cases like this
caching example, we provide an implementation in \rumpsteak using the Scribble
protocol shown in \cref{lst:CachingScribble}. We use Redis~\cite{Redis}, a
well-known in-memory database, for the cache. Each entry is indexed using a
combination of the request method (i.e.\ GET, POST, etc.), the path (e.g.\
\code{/index.html}) and the values of selected headers.

Moreover, to show that \rumpsteak can be used in real-world Rust applications,
our implementation integrates many popular libraries from Rust's \async/\await
ecosystem---Tokio~\cite{Tokio} for spawning concurrent asynchronous tasks,
Hyper~\cite{Hyper} for interfacing with HTTP and Fred~\cite{Fred} for
communicating with Redis. We distribute our implementation as a command-line
tool which can be used in practice as an HTTP cache.


==> arxiv/sections/conclusion_related.tex <==
\section{Conclusion and Related Work}
\label{sec:Related}

There are a vast number of studies on session types, some of which are
implemented in programming languages~\cite{Ancona2016} and tools~\cite{Gay2017}.
The top-down approach using Scribble~\cite{ScribbleWebsite,Yoshida2013,NuScr} we
presented in this paper has been implemented for a number of other programming
languages such as
Java~\cite{Hu2016,kouzapas_typechecking_2018,hu_explicit_2017},
Go~\cite{Castro2019}, TypeScript~\cite{Miu2021}, Scala~\cite{Scalas2017},
MPI-C~\cite{ng_protocols_2015}, F\#~\cite{Neykova2018}, F$\star$~\cite{Zhou2020}
and Actor DSL~\cite{harvey_multiparty_2021} to ensure \emph{correctness by
  construction}. Several implementations use an EFSM-based approach to generate
APIs from Scribble for target programming languages such
as~\cite{Hu2016,hu_explicit_2017,Neykova2018,Castro2019,Zhou2020,Miu2021,Scalas2017},
but none are integrated with \amr like \rumpsteak.

\rumpsteak provides three approaches for gaining \emph{efficiency} and ensuring
\emph{deadlock-freedom} in message-passing Rust applications: (1) the
\emph{top-down} approach for ensuring \emph{correctness/safety by construction}
and maximising \emph{asynchrony} with local analysis; (2) the \emph{bottom-up}
approach using global analysis on a set of FSMs; and (3) the \emph{hybrid}
approach, which combines inference with local analysis. All three approaches are
backed by \rumpsteak's API (described in \cref{sec:Overview}), which uses Rust's
affine type system to ensure protocol compliance.

Note that \rumpsteak is the first framework (for any programming
langauge) which enables the bottom-up (by integrating 
with \kmc~\cite{Lange2019}) and the hybrid approaches. 

\begin{description}
  \item[Rust session type implementations.]
    We closely compared the performance and expressiveness of \rumpsteak with
    three existing works in \cref{sec:Evaluation}:
    \begin{enumerate*}[label=\textbf{(\arabic*)}]
      \item \sesh~\cite{Kokke2019}, a synchronous implementation of binary
      session types;
      \item \ferrite~\cite{Chen2021}, an implementation of shared binary session
      types~\cite{Balzer2017} supporting asynchronous execution; and
      \item \multicrusty~\cite{Lagaillardie2020}, a synchronous \mpst
      implementation based on \sesh.
    \end{enumerate*}

    Of these previous implementations, only \multicrusty can also support \mpst
    with deadlock-freedom. However, to represent a multiparty session,
    \multicrusty requires defining a tuple of binary sessions for each role as
    well as their order of use. This leads to a more complex and less intuitive
    API than \rumpsteak's. Our API requires fewer definitions and is also both
    more expressive and performant (see \cref{sec:Evaluation}).

    \rumpsteak and \ferrite support asynchronous execution which is more
    efficient than the synchronous and blocking communication used by \sesh and
    \multicrusty. However, only \rumpsteak supports Rust's idiomatic
    \async/\await syntax. \ferrite instead requires nesting sequential
    communication, which is more verbose and less efficient. Iteration cannot be
    easily expressed (see~\cref{sec:Evaluation}) and it requires stricter
    compile-time concurrency guarantees than \rumpsteak. We do not compare
    directly against~\cite{Jespersen2015} (another synchronous implementation of
    binary session types) as this uses an older edition of Rust and has several
    limitations already discussed in~\cite{Lagaillardie2020,Kokke2019}.

    \rumpsteak can perform \amr, which is not possible in any of these existing
    implementations. Combined with its straightforward design and use of
    asynchronous execution, we found that it is therefore much more efficient
    than all previous work. It has around 14.5x, 3.2x and 1.9x greater
    throughput than the next fastest implementation in the stream, double
    buffering and FFT protocols respectively. \rumpsteak can also compete with a
    popular Rust implementation in the FFT benchmark, achieving the same
    throughput for large input sizes.

    Recent work~\cite{Duarte2021} builds a DSL to offer protocol conformance for
    Rust, supported by typestates. They do not yet explore combining the DSL
    with communication channels like \rumpsteak and
    \cite{Jespersen2015,Lagaillardie2020,Kokke2019,Balzer2017}. If this is
    achieved, it would be interesting to integrate session type tooling with
    their DSL and compare this with \rumpsteak.

  \item[Verification of asynchronous subtyping.] Interest in \amr has grown
    recently, both in theory and practice. An extension of the Iris framework,
    Actris~\cite{Hinrichsen_sessions_2021}, formalises a variant of binary
    asynchronous subtyping, which is in turn implemented in the Coq proof
    assistant. The asynchronous session subtyping defined
    in~\cite{Chen2017,Ghilezan2021} is \emph{precise} but was shown to be
    undecidable, even for binary sessions \cite{Lange2017,Bravetti2018}. Hence,
    in general, checking $\efsm_i' \leq \efsm_i$ is undecidable. Various limited
    classes of session types for which $\efsm_i' \leq \efsm_i$ is decidable
    \cite{Bravetti2019,Bravetti2017,Lange2017,CastroPerez2020} are proposed but
    they are not applicable to our use cases since \textbf{(1)} the relations in
    \cite{Bravetti2019,Bravetti2018,Lange2017} are \emph{binary} and the same
    limitations do not work for multiparty sessions; and \textbf{(2)} the
    relation in \cite[Def.~6.1]{CastroPerez2020} does not handle subtyping
    across unrolling recursions, e.g.\ the relation is inapplicable to the
    double buffering algorithm~\cite{Huang2002} (see \cite[Remark
      8.1]{CastroPerez2020}).

    Our new algorithm for asynchronous optimisation is \emph{terminating} (see
    \cref{thm:Termination}), \emph{sound} (see \cref{thm:Soundness}) and capable
    of verifying optimisations in a range of classical examples (see
    \cref{sec:Evaluation}). It is also more performant than a global analysis
    based on $k$-MC, and an existing 2-party sound algorithm~\cite{Bravetti2019}
    (see \cref{sec:Evaluation}). This is because our algorithm is implemented
    efficiently (see \cref{sec:AlgorithmImplementation}) and can often execute
    in linear rather than exponential time (see \cref{thm:Complexity}).

  \item[Deadlock detection.] There is also recent
    progress~\cite{Qin2020Detector,Qin2020} on static deadlock detection in Rust
    by tracking locks and unlocks in Rust's intermediate representation
    (MIR)~\cite{RustMIR}. This targets shared memory, rather than
    message-passing applications, and does not attempt safety by construction.
    In future work, we could also analyse the MIR directly in \rumpsteak,
    replacing the use of our API. However, it is difficult to identify
    concurrency primitives in the MIR (this would be made harder with
    \async/\await); \cite{Qin2020Detector} currently supports only three
    concurrent data structures from Rust's ecosystem.
\end{description}


==> arxiv/sections/evaluation.tex <==
\begin{figure*}
  \centering
  \sffamily\footnotesize
  \pgfplotslegendfromname{pgfplots:Runtime}
  \begin{tikzpicture}[every axis plot/.append style={thick}]
    \tikzset{mark options={mark size=1pt}}
    \begin{groupplot}[
        group style={group size=3 by 1},
        height=4cm,
        width=6.5cm
      ]
      \nextgroupplot[
        title=\textit{Streaming},
        xlabel=Number of values transferred (\(n\)),
        ylabel=Throughput (\(n\)/\(\mu\)s),
        xtick distance=10,
      ]
      \addplot[solid,mark=square*,color=primary,every mark/.append style={solid, fill=primary!30}] coordinates {
          (10,0.019389)
          (20,0.028142)
          (30,0.034193)
          (40,0.036566)
          (50,0.040315)
        };
      \addplot[dashed,mark=square*,color=secondary,every mark/.append style={solid, fill=secondary!30}] coordinates {
          (10,0.011678)
          (20,0.014325)
          (30,0.015160)
          (40,0.016072)
          (50,0.016577)
        };
      \addplot[densely dotted,mark=square*,color=tertiary,every mark/.append style={solid, fill=tertiary!30}] coordinates {
          (10,0.011386)
          (20,0.012994)
          (30,0.013463)
          (40,0.013671)
          (50,0.014126)
        };
      \addplot[dashed,mark=*,color=quinary,every mark/.append style={solid, fill=quinary!30}] coordinates {
          (10,0.202587)
          (20,0.336988)
          (30,0.427489)
          (40,0.488886)
          (50,0.545378)
        };
      \addplot[densely dotted,mark=*,color=senary,every mark/.append style={solid, fill=senary!30}] coordinates {
          (10,0.215583)
          (20,0.356978)
          (30,0.437795)
          (40,0.517468)
          (50,0.583366)
        };
      \nextgroupplot[
        title={\textit{Double Buffering}~\cite{CastroPerez2020,Huang2002}},
        xlabel=Number of values in each buffer (\(n\)),
        xtick distance=2500,
        ytick distance=20,
        scaled x ticks=false
      ]
      \addplot[solid,mark=square*,color=primary,every mark/.append style={solid, fill=primary!30}] coordinates {
          (2500,6.929567)
          (5000,13.138401)
          (7500,18.739983)
          (10000,24.103215)
          (12500,28.609966)
        };
      \addplot[dashed,mark=square*,color=secondary,every mark/.append style={solid, fill=secondary!30}] coordinates {
          (2500,5.675414)
          (5000,11.254181)
          (7500,16.187341)
          (10000,20.481378)
          (12500,25.050058)
        };
      \addplot[densely dotted,mark=square*,color=tertiary,every mark/.append style={solid, fill=tertiary!30}] coordinates {
          (2500,7.617643)
          (5000,14.649028)
          (7500,20.429845)
          (10000,25.506427)
          (12500,29.629025)
        };
      \addplot[dashed,mark=*,color=quinary,every mark/.append style={solid, fill=quinary!30}] coordinates {
          (2500,27.704354)
          (5000,44.154722)
          (7500,56.813002)
          (10000,67.595301)
          (12500,75.848611)
        };
      \addplot[densely dotted,mark=*,color=senary,every mark/.append style={solid, fill=senary!30}] coordinates {
          (2500,32.340989)
          (5000,50.126532)
          (7500,67.884430)
          (10000,82.039366)
          (12500,96.010424)
        };
      \nextgroupplot[
        title={\textit{FFT}~\cite{CastroPerez2020}},
        xlabel=Number of columns (\(n\)),
        xtick distance=1000,
        ytick distance=2,
        legend columns=-1,
        legend entries={\sesh,\multicrusty,\ferrite,\rustfft,\rumpsteak,\rumpsteak (optimised)},
        legend style={draw=none,column sep=5pt},
        legend to name=pgfplots:Runtime
      ]
      \addplot[solid,mark=square*,color=primary,every mark/.append style={solid, fill=primary!30}] coordinates {
          (1000,0.551154)
          (2000,1.050958)
          (3000,1.510567)
          (4000,1.935263)
          (5000,2.303627)
        };
      \addplot[dashed,mark=square*,color=secondary,every mark/.append style={solid, fill=secondary!30}] coordinates {
          (1000,0.810134)
          (2000,1.515538)
          (3000,2.163629)
          (4000,2.783617)
          (5000,3.261020)
        };
      \addplot[densely dotted,mark=square*,color=tertiary,every mark/.append style={solid, fill=tertiary!30}] coordinates {
          (1000,1.458279)
          (2000,2.513855)
          (3000,3.496405)
          (4000,4.198723)
          (5000,4.811375)
        };
      \addplot[solid,mark=*,color=quaternary,every mark/.append style={solid, fill=quaternary!30}] coordinates {
          (1000,9.320778)
          (2000,9.313359)
          (3000,9.333569)
          (4000,9.336939)
          (5000,9.323199)
        };
      \addplot[dashed,mark=*,color=quinary,every mark/.append style={solid, fill=quinary!30}] coordinates {
          (1000,5.038554)
          (2000,7.206404)
          (3000,8.421026)
          (4000,9.262763)
          (5000,9.316716)
        };
      \addlegendimage{densely dotted,mark=*,color=senary,every mark/.append style={solid, fill=senary!30}};
    \end{groupplot}
    \path (current bounding box.north)--++(0,5pt);
  \end{tikzpicture}
  \caption{Benchmarking \rumpsteak's runtime performance against previous work in Rust (raw data in \inApp{sec:RuntimeData}).}
  \label{fig:RuntimeBenchmarks}
\end{figure*}

\section{Evaluation}
\label{sec:Evaluation}

In this section, we evaluate how \rumpsteak performs with respect to existing
tools. First, in \cref{sec:RuntimeEvaluation}, we evaluate the runtime
performance of (multiparty) programs written in \rumpsteak versus the same
benchmarks implemented using other Rust session type tools. In the spirit of
Rust, this runtime performance is of particular significance for developers.
Secondly, in \cref{sec:eval_async_verif}, we evaluate how \rumpsteak's
verification of message reordering (our subtyping algorithm) scales compared to
existing verification tools. Although not a runtime cost, subtyping is known to
be a computationally challenging problem that often scales poorly.

\subsection{Session-Based Rust Implementations}
\label{sec:RuntimeEvaluation}

We compare \rumpsteak's runtime against three other session type implementations
in Rust:
\begin{enumerate*}[label=\textbf{(\arabic*)}]
  \item \sesh~\cite{Kokke2019}, a synchronous implementation of binary session
  types;
  \item \ferrite~\cite{Chen2021}, an implementation of shared binary session
  types~\cite{Balzer2017} supporting asynchronous execution; and
  \item \multicrusty~\cite{Lagaillardie2020}, a synchronous \mpst implementation
  based on \sesh.
\end{enumerate*}

We perform a series of benchmarks shown in \cref{fig:RuntimeBenchmarks}. We
execute these using an 16-core AMD Opteron\textsuperscript{TM} 6200 Series CPU @
2.6GHz with hyperthreading, 128GB of RAM, Ubuntu 18.04.5 LTS and Rust Nightly
2021-07-06. We use version 0.3.5 of the Criterion.rs library~\cite{Criterion} to
perform microbenchmarking and a \emph{multi-threaded} asynchronous runtime from
version 1.11.0 of the Tokio library~\cite{Tokio}.

\begin{description}
  \item[Streaming.] This protocol has two participants, a source \ppt{s} and a sink
    \ppt{t}, with a combination of recursion and choice. As stated previously, its global type
    $\gt_\textsf{ST}$ is given as
    \begin{equation*}
      \gt_\textsf{ST} = \gtrec{x}\gtmsg{t}{s}{\mathit{ready}.\gtmsg{s}{t}{
          \mathit{value}.\gtvar{x}, \quad
          \mathit{stop}.\gtend
        }}
    \end{equation*}
    We benchmark the protocol by varying the number of \(\mathit{value}\)s that
    are sent before the exchange \(\mathit{stop}\)s. We use \amr to create an
    optimised version for \rumpsteak: if the source knows it will send at least
    \(n\) \(\mathit{value}\)s before \(\mathit{stop}\)ping, then these messages
    can be \emph{unrolled} and sent all at once---only receiving
    \(\mathit{ready}\) from the sink after sending all \(n\)
    \(\mathit{value}\)s. For benchmarking, we unroll the first 5
    \(\mathit{value}\)s in the optimised version.

    Our results show \rumpsteak reaches around 14.5x the throughput of other
    implementations. At first, it is limited by channel creation overheads, the
    cost of which becomes less significant as more messages are sent. The
    throughput levels off as message passing overheads become the bottleneck.
    The optimised version eases this overhead, as the source is less frequently
    blocked on receiving \(\mathit{ready}\) from the sink---this effect could be
    increased by unrolling more messages.

    \sesh and \multicrusty have much lower throughputs since they use more
    expensive synchronous communication. These implementations also create a new
    channel for each interaction. This causes their throughput to stay constant
    as there are fewer one-time costs to spread than in \rumpsteak.
    Interestingly, \ferrite performs similarly to \sesh and \multicrusty,
    despite employing asynchronous execution like \rumpsteak. This is because
    its design requires that the source and sink are implemented using
    \emph{recursion} rather than \emph{iteration}. \ferrite also requires
    particularly strong safety requirements at compile time. Therefore, the
    sink's output buffer must be guarded with a mutex instead of being accessed
    directly.

  \item[Double Buffering.] We benchmark our running example by performing only
    two iterations. This allows for both of the kernel's buffers to be filled
    and, importantly, for the protocol to terminate. \sesh and \ferrite do not
    support \mpst so their implementations use binary session types between
    pairs of participants. This approach does \emph{not} provide the same safety
    as \mpst and so we cannot verify deadlock-freedom as we can in \multicrusty
    and \rumpsteak (see \cref{tab:Expressiveness}).

    We parameterise the size of the buffers and measure the throughput.
    Performance is similar to that of the stream benchmark; \rumpsteak's
    throughput reaches around 3.2x that of the others. Moreover, we confirm the
    intuition described in \cref{sec:Introduction}. Increasing the size of the
    buffers does generally improve throughput. However, it remains limited when
    only a single buffer can be used at once. \cref{fig:RuntimeBenchmarks} shows
    that optimising the kernel as described in \cref{sec:Overview} increases the
    throughput since the source and sink operate on different buffers at once.

  \item[FFT.] The fast Fourier transform (FFT) is an algorithm for computing
    the discrete Fourier transform of a vector. We take \(n \times 8\)
    \emph{matrices}, where the FFT is computed on each column to produce a new,
    transformed matrix, and implement the Cooley-Tukey FFT algorithm which
    divides the problem into---in our case---eight. Each of these problems can
    be solved independently by different processes, which communicate with one
    another using message passing. The exchanges between participants are
    described in \cite[Fig. 7]{CastroPerez2020}.

    We choosed to use FFT as a benchmark as it is a standard problem with
    numerous implementations, and we can therefore compare implementations
    based on MPST with actual high-optimised implementations.

    We implement a concurrent version of the algorithm in \sesh, \ferrite,
    \multicrusty and \rumpsteak, which uses eight processes. Each process works
    on an array of \(n\) inputs, representing one column. Arithmetic operations
    are performed in a pairwise fashion on two of these arrays.

    We use the same approach as in the double buffering protocol to write the
    binary implementations for \sesh and \ferrite. Interestingly, to represent
    this as a sequence of binary sessions, we require additional synchronisation
    of all participants at each stage of the protocol. While we can perform \amr
    to \rumpsteak's version, in practice we found that this does not have much
    effect since the protocol is already heavily synchronised so cannot progress
    any faster.

    We benchmark the protocol by varying the number of columns in the matrix. We
    also compare these implementations with the most downloaded open-source Rust
    FFT implementation, \rustfft~\cite{RustFFT}. \rustfft does not use
    concurrency and computes the FFT of a matrix by iteratively performing the
    Cooley-Tukey algorithm on each column.

    \ferrite performs better than before since its FFT implementation does not
    suffer from the limitations explained previously. Like \rumpsteak, it
    benefits from the use of asynchronous execution, although the additional
    synchronisation from representing the problem as a set of binary sessions
    causes \rumpsteak's throughput to remain around 1.9x greater.

    Most excitingly, \rumpsteak achieves \rustfft's throughput for large
    matrices. \rustfft's implementation is highly tuned for low-level efficiency
    and does not incur any overheads associated with message passing. Moreover,
    asynchronous executors are generally designed for higher-level tasks such as
    networking; MPI-based communication~\cite{MPI} would more likely be used to
    parallelise this problem in practice. Therefore, we think it impressive that
    even a basic parallel implementation using \rumpsteak can reach the same
    performance as a state-of-the-art sequential implementation.

    \begin{table*}
      \centering
      \caption{Expressiveness of \rumpsteak compared to previous work.}
      \label{tab:Expressiveness}
      \sffamily\footnotesize
      \setlength{\tabcolsep}{6pt}
      \begin{tabular}{lc|cccc|ccc|c|cc}
        \toprule
        Protocol                                                    & \(n\) & \feat{C} & \feat{R} & \feat{IR} & \feat{AMR} & \sesh  & \ferrite & \multicrusty & \rumpsteak & \kmc   & \concur \\
        \midrule
        Two Adder~\cite{NuScr}                                      & 2     & \tick    & \tick    &           &            & \ftick & \ftick   & \ftick       & \ftick     & \ftick & \ftick  \\
        Three Adder                                                 & 3     &          &          &           &            & \htick & \htick   & \ftick       & \ftick     & \ftick & \cross  \\
        Streaming                                                   & 2     & \tick    & \tick    &           &            & \ftick & \ftick   & \ftick       & \ftick     & \ftick & \ftick  \\
        Optimised Streaming                                         & 2     & \tick    & \tick    &           & \tick      & \cross & \cross   & \cross       & \ftick     & \ftick & \ftick  \\
        Ring~\cite{CastroPerez2020}                                 & 3     &          & \tick    & \tick     &            & \htick & \htick   & \ftick       & \ftick     & \ftick & \cross  \\
        Optimised Ring~\cite{CastroPerez2020}                       & 3     &          & \tick    & \tick     & \tick      & \htick & \htick   & \htick       & \ftick     & \ftick & \cross  \\
        Ring With Choice~\cite{CastroPerez2020}                     & 3     & \tick    & \tick    & \tick     &            & \htick & \htick   & \ftick       & \ftick     & \ftick & \cross  \\
        Optimised Ring With Choice~\cite{CastroPerez2020}           & 3     & \tick    & \tick    & \tick     & \tick      & \htick & \htick   & \htick       & \ftick     & \ftick & \cross  \\
        Double Buffering~\cite{CastroPerez2020}                     & 3     &          & \tick    & \tick     &            & \htick & \htick   & \ftick       & \ftick     & \ftick & \cross  \\
        Optimised Double Buffering~\cite{CastroPerez2020,Huang2002} & 3     &          & \tick    & \tick     & \tick      & \cross & \cross   & \cross       & \ftick     & \ftick & \cross  \\
        Alternating Bit~\cite{Lange2019,AlternatingBit}             & 2     & \tick    & \tick    & \tick     &            & \htick & \htick   & \htick       & \ftick     & \ftick & \ftick  \\
        Elevator~\cite{Lange2019,Bouajjani2018}                     & 3     & \tick    & \tick    & \tick     & \tick      & \cross & \cross   & \cross       & \ftick     & \ftick & \cross  \\
        FFT~\cite{CastroPerez2020}                                  & 8     &          &          &           &            & \htick & \htick   & \ftick       & \ftick     & \ftick & \cross  \\
        Optimised FFT~\cite{CastroPerez2020}                        & 8     &          &          &           & \tick      & \cross & \cross   & \cross       & \ftick     & \ftick & \cross  \\
        Authentication~\cite{Neykova2013}                           & 3     & \tick    &          &           &            & \htick & \htick   & \ftick       & \ftick     & \ftick & \cross  \\
        Client-Server Log~\cite{Lagaillardie2020}                   & 3     & \tick    & \tick    & \tick     &            & \htick & \htick   & \ftick       & \ftick     & \ftick & \cross  \\
        Hospital~\cite{Bravetti2019}                                & 2     & \tick    & \tick    & \tick     & \tick      & \cross & \cross   & \cross       & \htick     & \cross & \ftick  \\
        \bottomrule
      \end{tabular} \\[4pt]
      \footnotesize
      \(n\)\; Number of participants \quad \feat{C}\; Choice \quad \feat{R}\; Recursion \quad \feat{IR}\; Infinite recursion \quad \feat{AMR}\; Asynchronous message reordering \\[2pt]
      \ftick\; Expressible \quad \htick\; Expressible using endpoint types
      (but without deadlock-freedom guarantee) \quad \cross\; Not expressible
    \end{table*}

  \item[Expressiveness.] \cref{tab:Expressiveness} discusses the expressiveness
    of \rumpsteak compared with \sesh, \ferrite and \multicrusty. Since \sesh
    and \ferrite support only binary session types, they are unable to guarantee
    deadlock-freedom in protocols with more than two participants. \multicrusty
    has greater expressiveness than \sesh and \ferrite since it implements \mpst
    but, unlike \rumpsteak, still cannot ensure deadlock-freedom for protocols
    optimised using \amr. In addition, many optimisations, like the ones we have
    benchmarked, break duality between pairs of participants so are not
    expressible at all by \sesh, \ferrite and \multicrusty. Meanwhile, our
    powerful API and new subtyping algorithm allow \rumpsteak to express many
    examples using \amr.
\end{description}

\subsection{Verifying Asynchronous Message Reordering}
\label{sec:eval_async_verif}

We perform a second set of benchmarks, shown in \cref{fig:SubtypingBenchmarks},
to evaluate \rumpsteak's asynchronous subtyping algorithm. We compare it against
\begin{enumerate*}[label=\textbf{(\arabic*)}]
  \item \concur~\cite{Bravetti2019}, a sound subtyping algorithm defined for
  \emph{binary} session types only; and
  \item \kmc~\cite{Lange2019}, an algorithm for directly checking the
  compatibility of a set of FSMs without the need for a global type.
  Compatibility is checked up to a bound \(k\) on the size of each process'
  asynchronous queue.
\end{enumerate*}
We note that neither \concur nor \kmc provide a runtime framework like
\rumpsteak does, they are used only to verify the \amr.

\begin{figure*}
	\centering
	\sffamily\footnotesize
	\pgfplotslegendfromname{pgfplots:Subtyping}
	\begin{tikzpicture}[every axis plot/.append style={thick}]
		\tikzset{mark options={mark size=1pt}}
		\begin{groupplot}[
				group style={group size=4 by 1},
				height=4cm,
				width=4.8cm,
				ymode=log,
				ytick distance=10
			]
			\nextgroupplot[
				title=\textit{Streaming},
				xlabel=Number of unrolls ($n$),
				ylabel=Running time (\(\log \text{s}\)),
				legend columns=-1,
				legend entries={\concur,\kmc,\rumpsteak},
				legend style={draw=none,column sep=5pt},
				legend to name=pgfplots:Subtyping
			]
			\addplot[solid,mark=square*,color=primary,every mark/.append style={solid, fill=primary!30}] coordinates {
				(0,0.003476)
				(10,0.008556)
				(20,0.020673)
				(30,0.041673)
				(40,0.076425)
				(50,0.127865)
				(60,0.198541)
				(70,0.292471)
				(80,0.422571)
				(90,0.583863)
				(100,0.767426)
			};
			\addplot[dashed,mark=square*,color=secondary,every mark/.append style={solid, fill=secondary!30}] coordinates {
				(0,0.005504)
				(10,0.019316)
				(20,0.057417)
				(30,0.142145)
				(40,0.276446)
				(50,0.496929)
				(60,0.805577)
				(70,1.233327)
				(80,1.780778)
				(90,2.475443)
				(100,3.349204)
			};
			\addplot[densely dotted,mark=*,color=quinary,every mark/.append style={solid, fill=quinary!30}] coordinates {
				(0,0.001872)
				(10,0.001899)
				(20,0.001848)
				(30,0.001906)
				(40,0.001874)
				(50,0.002080)
				(60,0.002083)
				(70,0.002064)
				(80,0.002178)
				(90,0.002190)
				(100,0.002249)
			};
			\nextgroupplot[
				title={\textit{Nested Choice}~\cite[Fig. 3]{Chen2017}},
				xlabel=Number of levels ($n$),
				xtick distance=1
			]
			\addplot[solid,mark=square*,color=primary,every mark/.append style={solid, fill=primary!30}] coordinates {
				(1,0.002295)
				(2,0.004504)
				(3,0.016347)
				(4,0.224858)
				(5,4.692525)
			};
			\addplot[dashed,mark=square*,color=secondary,every mark/.append style={solid, fill=secondary!30}] coordinates {
				(1,0.006554)
				(2,0.014901)
				(3,0.072423)
				(4,1.515528)
				(5,41.688068)
			};
			\addplot[densely dotted,mark=*,color=quinary,every mark/.append style={solid, fill=quinary!30}] coordinates {
				(1,0.000702)
				(2,0.000755)
				(3,0.001745)
				(4,0.007656)
				(5,0.157548)
			};
			\nextgroupplot[
				title={\textit{Ring}~\cite{CastroPerez2020}},
				xlabel=Number of participants ($n$)
			]
			\addplot[dashed,mark=square*,color=secondary,every mark/.append style={solid, fill=secondary!30}] coordinates {
				(2,0.004007)
				(4,0.007239)
				(6,0.011806)
				(8,0.018822)
				(10,0.024842)
				(12,0.049232)
				(14,0.102257)
				(16,0.191078)
				(18,0.340262)
				(20,0.570656)
				(22,0.913412)
				(24,1.391075)
				(26,2.042452)
				(28,2.918943)
				(30,4.099072)
			};
			\addplot[densely dotted,mark=*,color=quinary,every mark/.append style={solid, fill=quinary!30}] coordinates {
				(2,0.000675)
				(4,0.000731)
				(6,0.000701)
				(8,0.000835)
				(10,0.000757)
				(12,0.000777)
				(14,0.000744)
				(16,0.000813)
				(18,0.000817)
				(20,0.000766)
				(22,0.000911)
				(24,0.000737)
				(26,0.000752)
				(28,0.000732)
				(30,0.000769)
			};
			\nextgroupplot[
				title={\textit{\(k\)-Buffering}~\cite{CastroPerez2020,Huang2002}},
				xlabel=Number of unrolls ($n$)
			]
			\addplot[dashed,mark=square*,color=secondary,every mark/.append style={solid, fill=secondary!30}] coordinates {
				(0,0.004825)
				(5,0.007668)
				(10,0.013613)
				(15,0.018770)
				(20,0.031376)
				(25,0.054910)
				(30,0.080879)
				(35,0.122315)
				(40,0.170533)
				(45,0.236354)
				(50,0.305749)
				(55,0.406071)
				(60,0.506069)
				(65,0.639521)
				(70,0.773931)
				(75,0.954399)
				(80,1.127240)
				(85,1.359600)
				(90,1.571745)
				(95,1.869339)
				(100,2.111687)
			};
			\addplot[densely dotted,mark=*,color=quinary,every mark/.append style={solid, fill=quinary!30}] coordinates {
				(0,0.000630)
				(5,0.000747)
				(10,0.000705)
				(15,0.000667)
				(20,0.000825)
				(25,0.000718)
				(30,0.000760)
				(35,0.000853)
				(40,0.000802)
				(45,0.000792)
				(50,0.000916)
				(55,0.000882)
				(60,0.000959)
				(65,0.001028)
				(70,0.001057)
				(75,0.001045)
				(80,0.001125)
				(85,0.001120)
				(90,0.001164)
				(95,0.001156)
				(100,0.001234)
			};
		\end{groupplot}
		\path (current bounding box.north)--++(0,5pt);
	\end{tikzpicture}
	\caption{Benchmarking \rumpsteak's subtyping performance against previous work  (raw data in \inApp{sec:VerificationData}).}
	\label{fig:SubtypingBenchmarks}
\end{figure*}


We benchmark with the same machine as before. \concur and \kmc are written in
Haskell so we must run each tool's binary rather than simply timing Rust
functions. We, therefore, provide a command-line for \rumpsteak's subtyping
algorithm so it is comparable with these other tools. \rumpsteak's binary is
compiled with Rust 1.54.0 and we use Hyperfine~\cite{Hyperfine} to compare the
execution time for each tool.

\begin{description}
  \item[Streaming (from \cref{sec:RuntimeEvaluation}).] We vary \(n\), the number
    of \(\mathit{value}\)s we unroll. Using \concur and \rumpsteak, we check
    that the optimised source is a subtype of its projected version and using
    \kmc, we check that the optimised source is compatible with the sink. Our
    results show that \rumpsteak scales significantly better than both \concur
    and \kmc. While all three implementations can verify up to 100 unrolls in
    under a second, the execution time taken by \concur and \kmc increases
    exponentially while \rumpsteak's remains mostly flat. This is consistent
    with our complexity analysis in \cref{thm:Complexity}, since unrolling more
    \(\mathit{value}\)s does not increase the branching factor of the subtype.

  \item[Nested choice.] We next consider a protocol from \citet[Fig.
      3]{Chen2017} containing nested choice. We perform this nesting up to a
    parameterised number of levels $n$ to increase the complexity.
    Specifically, we check that $\lt_n \leq \lt'_n$ where
    \begin{center}
      $\lt_0 = \lt'_0 = \tend$ \\
      $\lt_{n + 1}  = \tout{}\mathit{m}.(\tin{}\mathit{r}.\lt_n\ \&\ \tin{}\mathit{s}.\lt_n\ \&\ \tin{}\mathit{u}.\lt_n) \oplus \tout{}\mathit{p}.(\tin{}\mathit{r}.\lt_n\ \&\ \tin{}\mathit{s}.\lt_n)$        \\
      $\lt'_{n + 1} = \tin{}\mathit{r}.(\tout{}\mathit{m}.\lt'_n \oplus \tout{}\mathit{p}.\lt'_n \oplus \tout{}\mathit{q}.\lt'_n)\ \&\ \tin{}\mathit{s}.(\tout{}\mathit{m}.\lt'_n \oplus \tout{}\mathit{p}.\lt'_n)$
    \end{center}

    We find that \rumpsteak again performs more scalably than \concur and \kmc.
    Here, \rumpsteak's improved efficiency is significant---for five levels,
    \kmc takes around 40s while \rumpsteak requires only a fraction of a second.
    Nonetheless, we observe that \rumpsteak also exhibits exponential
    performance, in contrast to our stream benchmark. This is because our
    algorithm bounds recursion but not choice, causing an explosion in the paths
    to visit as the number of nested choices increases. This is also explained
    by our complexity analysis in \cref{thm:Complexity} since a greater number
    of nested choices increases the depth to which we must explore.

  \item[Ring~\cite{CastroPerez2020}.] We consider a ring protocol with a parameterised number of
    participants. Each participant (aside from the first, which initiates the
    protocol) receives a value from its preceding neighbour then sends a value
    to its succeeding neighbour. Providing that this receive is not dependent on
    the send, we can use \amr to send before receiving.

    We benchmark verifying this optimisation using both \kmc and \rumpsteak. In
    this case, we cannot use \concur since the protocol is multiparty. While
    \rumpsteak can verify each participant's subtype individually, \kmc must
    consider the entire protocol at once. Unsurprisingly, \kmc is significantly
    less scalable as its running time grows exponentially, whereas \rumpsteak's
    performance remains mostly constant.

  \item[\(k\)-buffering.] We extend the double buffering protocol to a
    parameterised number of buffers. We benchmark verifying the optimisation to
    the kernel discussed previously. Crucially, with a greater number of
    buffers, we can unroll a greater number of \(\text{ready}\) messages. We
    again compare only \kmc and \rumpsteak since the protocol is multiparty.
    Similarly to other benchmarks, \rumpsteak scales more efficiently than \kmc.

  \item[Expressiveness.] \cref{tab:Expressiveness} discusses the expressiveness
    of \rumpsteak's algorithm against \concur and \kmc (note again that \concur
    and \kmc only verify \amr and do not provide language implementations like
    \rumpsteak). As we discussed, \concur supports only 2 parties so cannot
    express many of the case studies. However, it can express some unbounded
    binary protocols that \rumpsteak and \kmc cannot, such as the hospital
    example~\cite[\textbf{\S~1}]{Bravetti2019}\footnote{Notice,
          for the case of \rumpsteak, that we can manually write the endpoints, and
          the framework checks the conformance to the protocol. However, \rumpsteak
          can not verify the \emph{deadlock-freedom} property of the protocol, hence
          the \emph{amber cross}.}. Unsurprisingly, \kmc's expressiveness in the
    table coincides with \rumpsteak's as \kmc with $k{=}\infty$ is equivalent
    to the liveness property induced by asynchronous multiparty
    subtyping~\cite[Theorem 7.3]{Ghilezan2021}. On the other hand, \kmc can
    verify a wider syntax of local FSMs than those corresponding to
    \cref{def:syntax}.
\end{description}


==> arxiv/sections/introduction.tex <==
\section{Introduction}
\label{sec:Introduction}

Rust is a statically-typed language designed for systems software development.
It is rapidly growing in popularity and has been voted ``most loved language''
over five years of surveys by Stack Overflow~\cite{StackOverflowSurvey}. Rust
aims to offer the safety of a high-level language without compromising on the
performance enjoyed by low-level languages. \emph{Message passing} over
\emph{typed channels} is common in concurrent Rust applications, where
(low-level) threads or (high-level) actors communicate efficiently and safely by
sending messages containing data.

To improve performance by maximising computation-communication
overlap~\cite{Choi2020,Sergent2018,Kim2012}, developers often wish to
arbitrarily change the order of sending and receiving messages---we will present
several examples of this technique, which we refer to as \emph{asynchronous
	message reordering} (\amr). Our challenge is to remedy communication errors such
as deadlocks, which can easily occur in message-passing applications,
particularly those that leverage \amr.

To achieve this, we introduce \rumpsteak: a framework for efficiently
coordinating message-passing processes in Rust using \emph{multiparty session
	types}. Session types~\cite{Honda1998,Takeuchi1994} (see \cite{Yoshida2020} for
a gentle introduction and~\cite{gay_behavioural_2017} for a more exhaustive one)
coordinate interactions through \emph{linearly typed channels}, that must be
used exactly once, ensuring \emph{protocol compliance} without deadlocks or
communication mismatches.

\paragraph{Current state of the art}
Since Rust's \emph{affine type system} is particularly well-suited to session
types by statically guaranteeing a linear usage of session channels, there are
several previous attempts at implementing session types in
Rust~\cite{Lagaillardie2020,Chen2021,Kokke2019,Jespersen2015}. However, their
current limitations prevent them from guaranteeing all four of
\emph{deadlock-freedom}, \emph{multiparty communication}, \emph{asynchronous
	execution} and \amr.

\paragraph{Our framework} We motivate the importance of each feature and explain
how \rumpsteak incorporates this.
\begin{description}
	\item[Deadlock-freedom.] One of the most important properties of concurrent/parallel systems
		is that their computations are not
                blocked. Deadlock-freedom in our context states that 
the system can always make a progress by exchanging messages, 
or properly terminate.

	\item[Multiparty communication.] Many of previous Rust 
		implementations~\cite{Chen2021,Kokke2019,Jespersen2015} support only
		\emph{binary} session types, which is limited to two party communication.
		On the other hand, the majority of real-world communication protocols consist of more than two participants. \rumpsteak therefore
		uses \emph{multiparty} session types (\mpst)~\cite{Honda2016,Honda2008}
		to ensure deadlock-freedom in protocols with any number of participants
		(or roles).

	\item[Asynchronous execution.] Most of previous Rust 
		implementations~\cite{Lagaillardie2020,Kokke2019,Jespersen2015} use
		\emph{synchronous} communication channels. This approach suffers from
		performance limitations since threads are \emph{blocked} while waiting
		to receive messages. \rumpsteak instead uses \emph{asynchronous}
		communication, where lightweight asynchronous tasks share a pool of
		threads. When one task is blocked, another's work can be scheduled in
		the meantime to prevent the wasting of computational resources.

		Although \cite{Chen2021} is also based on asynchronous communication,
		only \rumpsteak closely integrates with Rust's modern \async/\await
		syntax, allowing asynchronous programs to be written sequentially. To
		achieve this, asynchronous functions are annotated with \async, causing
		them to return \emph{futures}. Developers can \await calls to these
		functions, denoting that execution should continue elsewhere until a
		result is ready.

		\begin{figure*}
			\centering
			\sffamily\footnotesize
			$\boldsymbol{\gt}$ \; Global Type \qquad
			$\boldsymbol{\efsm}$ \; Finite State Machine (FSM) \qquad
			$\boldsymbol{\oefsm}$ \; Optimised FSM \qquad
			$\boldsymbol{\api}$ \; Rust API \qquad
			$\boldsymbol{\proc}$ \; Rust Process \\[.4cm]
			\begin{subfigure}[b]{0.3\textwidth}
				\centering
				\begin{tikzpicture}[
						x=.3cm, y=-.95cm, align=center, thick,
						font=\footnotesize\linespread{0.8}\selectfont, draw,
						minimum size=.55cm,
						>=to, node distance=.4cm,
						hand/.style={fill=primary!30, draw=primary, densely dotted, rounded corners},
						generated/.style={fill=secondary!30, draw=secondary, rounded corners},
						compat/.style={fill=tertiary!15, draw=none, rounded corners},
						kmc/.style={fill=quaternary!15, draw=none, rounded corners},
						subtype/.style={fill=quinary!15, draw=none, rounded corners}
					]
					\node [hand, inner sep=1mm] (G) at (4,0) {$\gt$};
					\node [below=of G] (GB) {};
					\node [inner sep=1mm, right=-0.1cm of GB] (LL) {$\ldots$};
					\node [generated, inner sep=1mm, left=of LL] (L2) {$\efsm_2$};
					\node [generated, inner sep=1mm, left=of L2] (L1) {$\efsm_1$};
					\node [generated, inner sep=1mm, right=of LL] (Ln) {$\efsm_n$};
					\node [hand, inner sep=1mm, below=.15cm of L1] (M1) {$\oefsm_1$};
					\node [hand, inner sep=1mm, below=.15cm of L2] (M2) {$\oefsm_2$};
					\node [inner sep=1mm, below=.15cm of LL] (MM) {$\ldots$};
					\node [hand, inner sep=1mm, below=.15cm of Ln] (Mn) {$\oefsm_n$};
					\node [generated, inner sep=1mm, below=.6cm of M1] (A1) {$\api_1$};
					\node [generated, inner sep=1mm, below=.6cm of M2] (A2) {$\api_2$};
					\node [inner sep=1mm, below=.6cm of MM] (AA) {$\ldots$};
					\node [generated, inner sep=1mm, below=.6cm of Mn] (An) {$\api_n$};
					\node [hand, inner sep=1mm, below=.15cm of A1] (P1) {$\proc_1$};
					\node [hand, inner sep=1mm, below=.15cm of A2] (P2) {$\proc_2$};
					\node [inner sep=1mm, below=.15cm of AA] (PP) {$\ldots$};
					\node [hand, inner sep=1mm, below=.15cm of An] (Pn) {$\proc_n$};

					\begin{scope}[on background layer]
						\node [subtype, fit=(L1)(M1)] (sub1) {};
						\node [subtype, fit=(L2)(M2)] (sub2) {};
						\node [subtype, fit=(Ln)(Mn)] (subn) {};
					\end{scope}
					\node [left=1mm of sub1, anchor=south, rotate=90] {Asynchronous\\Subtyping};

					\begin{scope}[on background layer]
						\node [compat, fit=(A1)(P1)] (compat1) {};
						\node [compat, fit=(A2)(P2)] (compat2) {};
						\node [compat, fit=(An)(Pn)] (compatn) {};
					\end{scope}
					\node [left=1mm of compat1, anchor=south, rotate=90] {Rust Typecheck};

					\draw [->] (G.south) to (L1);
					\draw [->] (G.south) to (L2);
					\draw [->] (G.south) to (LL);
					\draw [->] (G.south) to (Ln);
					\draw [->] (M1) to (A1);
					\draw [->] (M2) to (A2);
					\draw [->] (MM) to (AA);
					\draw [->] (Mn) to (An);
				\end{tikzpicture}
				\caption{Top-down}
				\label{fig:topdownapproach}
			\end{subfigure}\begin{subfigure}[b]{0.4\textwidth}
				\centering
				\begin{tikzpicture}[
						x=.3cm, y=-.95cm, align=center, thick,
						font=\footnotesize\linespread{0.8}\selectfont, draw,
						minimum size=.4cm,
						>=to, node distance=.4cm,
						hand/.style={fill=primary!30, draw=primary, densely dotted, rounded corners=4},
						generated/.style={fill=secondary!30, draw=secondary, rounded corners=4},
						compat/.style={fill=tertiary!15, draw=none, rounded corners},
						kmc/.style={fill=quaternary!15, draw=none, rounded corners},
						subtype/.style={fill=quinary!15, draw=none, rounded corners}
					]
					\matrix[column sep=.2cm]{
						\node[hand]  {};  &
						\node {User-Written};  &
						\node[generated] {}; &
						\node {Generated};   \\
					};
				\end{tikzpicture} \\[.3cm]
				\begin{tikzpicture}[
						x=.3cm, y=-.95cm, align=center, thick,
						font=\footnotesize\linespread{0.8}\selectfont, draw,
						minimum size=.55cm,
						>=to, node distance=.4cm,
						hand/.style={fill=primary!30, draw=primary, densely dotted, rounded corners},
						generated/.style={fill=secondary!30, draw=secondary, rounded corners},
						compat/.style={fill=tertiary!15, draw=none, rounded corners},
						kmc/.style={fill=quaternary!15, draw=none, rounded corners},
						subtype/.style={fill=quinary!15, draw=none, rounded corners}
					]
					\node [generated, inner sep=1mm] (M1) {$\oefsm_1$};
					\node [generated, inner sep=1mm, right=of M1] (M2) {$\oefsm_2$};
					\node [inner sep=1mm, right=of M2] (MM) {$\ldots$};
					\node [generated, inner sep=1mm, right=of MM] (Mn) {$\oefsm_n$};
					\node [hand, inner sep=1mm, below=.6cm of M1] (A1) {$\api_1$};
					\node [hand, inner sep=1mm, below=.6cm of M2] (A2) {$\api_2$};
					\node [inner sep=1mm, below=.6cm of MM] (AA) {$\ldots$};
					\node [hand, inner sep=1mm, below=.6cm of Mn] (An) {$\api_n$};
					\node [hand, inner sep=1mm, below=.15cm of A1] (P1) {$\proc_1$};
					\node [hand, inner sep=1mm, below=.15cm of A2] (P2) {$\proc_2$};
					\node [inner sep=1mm, below=.15cm of AA] (PP) {$\ldots$};
					\node [hand, inner sep=1mm, below=.15cm of An] (Pn) {$\proc_n$};

					\begin{scope}[on background layer]
						\node [kmc, fit=(M1)(Mn)] (kMC) {};
					\end{scope}
					\node [above=1mm of kMC, anchor=south] {$k$-Multiparty Compatibility~\cite{Lange2019}};

					\begin{scope}[on background layer]
						\node [compat, fit=(A1)(P1)] (compat1) {};
						\node [compat, fit=(A2)(P2)] (compat2) {};
						\node [compat, fit=(An)(Pn)] (compatn) {};
					\end{scope}
					\node [left=1mm of compat1, anchor=south, rotate=90] {Rust Typecheck};

					\draw [<-] (M1) to (A1);
					\draw [<-] (M2) to (A2);
					\draw [<-] (MM) to (AA);
					\draw [<-] (Mn) to (An);
				\end{tikzpicture}
				\caption{Bottom-up}
				\label{fig:bottomup}
			\end{subfigure}\begin{subfigure}[b]{0.3\textwidth}
				\centering
				\begin{tikzpicture}[
						x=.3cm, y=-.95cm, align=center, thick,
						font=\footnotesize\linespread{0.8}\selectfont, draw,
						minimum size=.55cm,
						>=to, node distance=.4cm,
						hand/.style={fill=primary!30, draw=primary, densely dotted, rounded corners},
						generated/.style={fill=secondary!30, draw=secondary, rounded corners},
						compat/.style={fill=tertiary!15, draw=none, rounded corners},
						kmc/.style={fill=quaternary!15, draw=none, rounded corners},
						subtype/.style={fill=quinary!15, draw=none, rounded corners}
					]
					\node [hand, inner sep=1mm] (G) at (4,0) {$\gt$};
					\node [below=of G] (GB) {};
					\node [inner sep=1mm, right=-0.1cm of GB] (LL) {$\ldots$};
					\node [generated, inner sep=1mm, left=of LL] (L2) {$\efsm_2$};
					\node [generated, inner sep=1mm, left=of L2] (L1) {$\efsm_1$};
					\node [generated, inner sep=1mm, right=of LL] (Ln) {$\efsm_n$};
					\node [generated, inner sep=1mm, below=.15cm of L1] (M1) {$\oefsm_1$};
					\node [generated, inner sep=1mm, below=.15cm of L2] (M2) {$\oefsm_2$};
					\node [inner sep=1mm, below=.15cm of LL] (MM) {$\ldots$};
					\node [generated, inner sep=1mm, below=.15cm of Ln] (Mn) {$\oefsm_n$};
					\node [hand, inner sep=1mm, below=.6cm of M1] (A1) {$\api_1$};
					\node [hand, inner sep=1mm, below=.6cm of M2] (A2) {$\api_2$};
					\node [inner sep=1mm, below=.6cm of MM] (AA) {$\ldots$};
					\node [hand, inner sep=1mm, below=.6cm of Mn] (An) {$\api_n$};
					\node [hand, inner sep=1mm, below=.15cm of A1] (P1) {$\proc_1$};
					\node [hand, inner sep=1mm, below=.15cm of A2] (P2) {$\proc_2$};
					\node [inner sep=1mm, below=.15cm of AA] (PP) {$\ldots$};
					\node [hand, inner sep=1mm, below=.15cm of An] (Pn) {$\proc_n$};

					\begin{scope}[on background layer]
						\node [subtype, fit=(L1)(M1)] (sub1) {};
						\node [subtype, fit=(L2)(M2)] (sub2) {};
						\node [subtype, fit=(Ln)(Mn)] (subn) {};
					\end{scope}
					\node [left=1mm of sub1, anchor=south, rotate=90] {Asynchronous\\Subtyping};

					\begin{scope}[on background layer]
						\node [compat, fit=(A1)(P1)] (compat1) {};
						\node [compat, fit=(A2)(P2)] (compat2) {};
						\node [compat, fit=(An)(Pn)] (compatn) {};
					\end{scope}
					\node [left=1mm of compat1, anchor=south, rotate=90] {Rust Typecheck};

					\draw [->] (G.south) to (L1);
					\draw [->] (G.south) to (L2);
					\draw [->] (G.south) to (LL);
					\draw [->] (G.south) to (Ln);
					\draw [<-] (M1) to (A1);
					\draw [<-] (M2) to (A2);
					\draw [<-] (MM) to (AA);
					\draw [<-] (Mn) to (An);
				\end{tikzpicture}
				\caption{Hybrid}
				\label{fig:hybridapproach}
			\end{subfigure}
			\caption{Workflow of the \rumpsteak framework (three approaches).}
			\label{fig:approaches}
		\end{figure*}

	\item[Asynchronous message reordering.] Our main contribution is offering
		\amr, which no existing work can provide while preserving deadlock-freedom.
		To motivate this, we introduce a running example of the \emph{double
			buffering} protocol~\cite{Huang2002}. Buffering is frequently used in
		multimedia applications where a continuous stream of data must be sent from
		a source (e.g.\ a graphics card) to a sink (e.g.\ a CPU). To prevent the
		source from being blocked while the sink is busy, it writes to a buffer,
		which is later read by the sink.

		\begin{figure}[h]
			\centering
			\sffamily\footnotesize
			\begin{tikzpicture}[
					x=11.5pt, y=-10pt, thick,
					copy/.style={
							{Circle[width=3pt, length=3pt]}-to,
							shorten <=-1.5pt, shorten >=-1.5pt
						},
					time/.style={-To, every node/.style={fill=white}}
				]
				\node[anchor=south, rotate=90] at (0,1) {Source};
				\node[anchor=south, rotate=90] at (0,4) {Buffers};
				\node[anchor=south, rotate=90] at (0,7) {Sink};

				% Single buffer
				\node[anchor=south] at (5,0) {\textit{Single Buffer}};
				\path[time] (.5,8.5) edge node {\textbf{Time}} (9.5,8.5);

				\draw[draw=none, fill=secondary!30, rounded corners] (.5,.5) rectangle ++(9,1);
				\draw[draw=none, fill=senary!30, rounded corners] (.5,6.5) rectangle ++(9,1);

				\draw[primary, fill=primary!30, rounded corners] (1.5,2) rectangle ++(1,2);
				\path[copy] (2,1) edge node {} (2,3);

				\draw[primary, fill=primary!30, rounded corners] (3.5,2) rectangle ++(1,2);
				\path[copy] (4,3) edge node {} (4,7);

				\draw[primary, fill=primary!30, rounded corners] (5.5,2) rectangle ++(1,2);
				\path[copy] (6,1) edge node {} (6,3);

				\draw[primary, fill=primary!30, rounded corners] (7.5,2) rectangle ++(1,2);
				\path[copy] (8,3) edge node {} (8,7);

				% Double buffer
				\node[anchor=south] at (15,0) {\textit{Double Buffer}};
				\path[time] (10.5,8.5) edge node {\textbf{Time}} (19.5,8.5);

				\draw[draw=none, fill=secondary!30, rounded corners] (10.5,.5) rectangle ++(9,1);
				\draw[draw=none, fill=senary!30, rounded corners] (10.5,6.5) rectangle ++(9,1);

				\draw[primary, fill=primary!30, rounded corners] (11.5,2) rectangle ++(1,2);
				\draw[quinary, fill=quinary!30, rounded corners] (11.5,4) rectangle ++(1,2);
				\path[copy] (12,1) edge node {} (12,3);

				\draw[primary, fill=primary!30, rounded corners] (13.5,2) rectangle ++(1,2);
				\draw[quinary, fill=quinary!30, rounded corners] (13.5,4) rectangle ++(1,2);
				\path[copy, bend left=70] (14,1) edge node {} (14,5);
				\path[copy, bend right=70] (14,3) edge node {} (14,7);

				\draw[primary, fill=primary!30, rounded corners] (15.5,2) rectangle ++(1,2);
				\draw[quinary, fill=quinary!30, rounded corners] (15.5,4) rectangle ++(1,2);
				\path[copy] (16,1) edge node {} (16,3);
				\path[copy] (16,5) edge node {} (16,7);

				\draw[primary, fill=primary!30, rounded corners] (17.5,2) rectangle ++(1,2);
				\draw[quinary, fill=quinary!30, rounded corners] (17.5,4) rectangle ++(1,2);
				\path[copy, bend left=70] (18,1) edge node {} (18,5);
				\path[copy, bend right=70] (18,3) edge node {} (18,7);
			\end{tikzpicture}
			\caption{Illustration of the double buffering protocol.}
			\label{fig:DoubleBuffering}
		\end{figure}

		We illustrate this effect in \cref{fig:DoubleBuffering}. With a single
		buffer, both the source and sink are constantly blocked as we cannot
		read and write simultaneously. However, adding a second buffer allows
		the source and sink to operate on different buffers at once so that (in
		the best case) they are never blocked and throughput can increase
		twofold.

		As we will see in \cref{sec:Overview}, the double buffering protocol
		takes advantage of \amr so it \emph{cannot} be expressed with standard
		\mpst theory~\cite{Honda2008}; communication with the source and sink
		are overlapped so both buffers can be accessed at once. The goal of this
		paper is to provide a method for ensuring that protocols optimised in
		this way preserve deadlock-freedom.
\end{description}

\paragraph{\rumpsteak framework} We achieve these features while allowing three
different approaches, summarised in \cref{fig:approaches}.

In the \textbf{top-down approach}, the developer writes a global type, which
describes the entire protocol (see \cref{sec:Overview} for an example). We
project this onto each participant to obtain a local finite state machine
(FSM), which describes the protocol from that participant's perspective.
Next, the developer uses \amr to propose optimised FSMs for each
participant. We \emph{locally} verify that each optimised FSM is compatible
with the projected one using an asynchronous subtyping algorithm. From each
optimised FSM, we generate an API so that the developer can write a Rust
process implementation. Our API uses Rust's type checker to ensure that
these processes conform to the protocol, and are therefore deadlock-free.

In the \textbf{bottom-up approach}, the developer manually writes an API and
process implementation for each participant. We derive the optimised FSMs
directly from these APIs and ensure that they are safe using
\emph{\(k\)-multiparty compatibility} (\kmc)~\cite{Lange2019}. \kmc globally
verifies that multiple FSMs are compatible with each other without using a
global type.

Finally, we propose a \textbf{hybrid approach} where the projected FSMs are
generated from a global type on one side (as in the top-down approach). On the
other side, the developer writes both the APIs and process implementations
directly, and we derive the optimised FSMs (as in the bottom-up approach). We
then \emph{locally} verify that the optimised FSMs are asynchronous subtypes of
the projected FSMs.

To summarise, our subtyping algorithm used in the top-down/hybrid approaches
\emph{locally} verifies the correctness of optimisations. This makes it far more
scalable than \kmc as we will see in \cref{sec:Evaluation}. These approaches are
also more intuitive to the developer since they use \emph{safety by
	construction}---it is much easier to write a global type than to determine why a
\kmc analysis has failed for a complex protocol.

\paragraph{Contribution and outline} In \cref{sec:Overview}, we give an overview
of the design and implementation of \rumpsteak. In \cref{sec:Theory}, we present
our new \emph{asynchronous subtyping algorithm} used to check that an optimised
FSM is correct. We prove our new algorithm is \emph{sound}
(\cref{thm:Soundness}) against the precise \mpst asynchronous subtyping
theory~\cite{Ghilezan2021} and \emph{terminates} (\cref{thm:Termination}), and
analyse its complexity (\cref{thm:Complexity}). In \cref{sec:Evaluation}, we
compare the performance and expressiveness of our framework with existing
work~\cite{Lagaillardie2020,Chen2021,Kokke2019,Lange2019,Bravetti2019}. We show
\begin{enumerate*}[label=\textbf{(\arabic*)}]
	\item \rumpsteak's runtime is faster and can express many more asynchronous
	protocols than other Rust
	implementations~\cite{Lagaillardie2020,Kokke2019,Chen2021}; and
	\item our subtyping algorithm is more efficient than existing
	algorithms~\cite{Lange2019,Bravetti2019}, confirming our complexity
	analysis.
\end{enumerate*}
\cref{sec:Related} discusses related work and concludes. The
\textbf{supplementary materials} available in the full
version~\cite{FullVersion} contain further examples and proofs of the theorems.
We include our source code and benchmarks in a \textbf{public GitHub
	repository}~\repository.


==> arxiv/sections/overview.tex <==
\section{Design and Implementation}
\label{sec:Overview}
This section presents \rumpsteak and explains its three workflows: a
\emph{top-down approach} using asynchronous subtyping, a \emph{bottom-up
  approach} using $k$-multiparty compatibility (\kmc)~\cite{Lange2019} and a
\emph{hybrid approach} combining the two.

\begin{figure*}
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \begin{lstlisting}[language=Scribble]
global protocol DoubleBuffering
    (role s, role k, role t) {
  rec loop {
    ready() from k to s;
    copy() from s to k;
    ready() from t to k;
    copy() from k to t;
    continue loop;
  }
}
\end{lstlisting}
    \caption{Scribble protocol description}
    \label{fig:example_scribble}
  \end{subfigure}\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \begin{tikzpicture}[>=to, -to, thick, font=\footnotesize, initial left, initial distance=1.5ex, initial text={}, state/.style={draw, circle, node distance=1cm and 1.6cm, inner sep=3pt}, every path/.style={every node/.style={fill=white}}]
      \node[state,initial] (1) {};
      \node[state] (2) [right=of 1] {};

      \path (1) edge[bend left] node {$\tin{k}\mathit{ready}$} (2);
      \path (2) edge[bend left] node {$\tout{k}\mathit{value}$} (1);
    \end{tikzpicture}

    \vspace{.4cm}
    \begin{tikzpicture}[>=to, -to, thick, font=\footnotesize, initial left, initial distance=1.5ex, initial text={}, state/.style={draw, circle, node distance=1cm and 1.6cm, inner sep=3pt}, every path/.style={every node/.style={fill=white}}]
      \node[state,initial] (1) {};
      \node[state] (2) [right=of 1] {};
      \node[state] (3) [below=of 2] {};
      \node[state] (4) [left=of 3] {};

      \path (1) edge node {$\tout{s}\mathit{ready}$} (2);
      \path (2) edge node[fill=none, sloped, anchor=north] {$\tin{s}\mathit{value}$} (3);
      \path (3) edge node {$\tin{t}\mathit{ready}$} (4);
      \path (4) edge node[fill=none, sloped, anchor=north] {$\tout{t}\mathit{value}$} (1);
    \end{tikzpicture}

    \vspace{.4cm}
    \begin{tikzpicture}[>=to, -to, thick, font=\footnotesize, initial left, initial distance=1.5ex, initial text={}, state/.style={draw, circle, node distance=1cm and 1.6cm, inner sep=3pt}, every path/.style={every node/.style={fill=white}}]
      \node[state,initial] (1) {};
      \node[state] (2) [right=of 1] {};

      \path (1) edge[bend left] node {$\tout{k}\mathit{ready}$} (2);
      \path (2) edge[bend left] node {$\tin{k}\mathit{value}$} (1);
    \end{tikzpicture}
    \caption{Projected FSMs for the source, the kernel and the sink}
    \label{fig:example_automata}
  \end{subfigure}\begin{subfigure}[b]{0.3\textwidth}
    \centering
    \begin{lstlisting}[language=Rust]
#[session]
struct Source(Receive<K, Ready,
  Send<K, Copy, Source>>);

#[session]
struct Kernel(Send<S, Ready,
	Receive<S, Copy,
	Receive<T, Ready,
	Send<T, Copy, Kernel>>>>);

#[session]
struct Sink(Send<K, Ready,
	Receive<K, Copy, Sink>>);
\end{lstlisting}
    \caption{Generated Rust code (excerpt)}
    \label{fig:example_rust}
  \end{subfigure}
  \caption{The three kinds of formats that are used in \rumpsteak.}
  \label{fig:rumpsteak_files}
\end{figure*}

\subsection{Top-Down Approach}
\label{sec:TopDown}

All three approaches result in the same final application, so we use the example
of the top-down workflow (\cref{fig:topdownapproach}) to give a  general
overview of \rumpsteak's implementation.

\paragraph{Two party protocol}
Before going into the details of the top-down approach, we first give an
informal insight into session types. As an example of a session type, we show
the global type for a streaming example, later introduced
in~\cref{sec:Evaluation}.
\begin{equation*}
  \gt_\textsf{ST} = \gtrec{x}\gtmsg{t}{s}{\mathit{ready}.\gtmsg{s}{t}{
      \mathit{value}.\gtvar{x}, \quad
      \mathit{stop}.\gtend
    }}
\end{equation*}
This type describes the streaming protocol from a global perspective,
and is read
as follows: participant \(\ppt{t}\) first sends \(\mathit{ready}\) to 
participant \(\ppt{s}\). Next,
\(\ppt{s}\) replies to \(\ppt{t}\) with two possible messages: either
\(\mathit{value}\) or \(\mathit{stop}\). In the latter case, the protocol
terminates (type \(\gtend\)). In the former case, the protocol continues with
\(\gtvar{x}\), which is a type variable that is bound by \(\gtrec{x}\), i.e. the
protocol starts over. 

\paragraph{Multiparty protocol}
In the remainder of this section, we use a slightly more
complex example (the double buffering protocol from
\cref{sec:Introduction}), 
which allows us to illustrate 
multiparty session types which can be verified in \rumpsteak.

In \rumpsteak, developers express global types syntactically with
Scribble~\cite{ScribbleWebsite,Yoshida2013} and we perform projection using
\nuscr~\cite{NuScr}. Scribble is a widely used and target-agnostic language for
describing multiparty protocols and \nuscr is a new lightweight and extensible
Scribble toolchain implemented in OCaml.

Once we have created a global type, we use an algorithm to project this onto
each participant. In practice, this results in an FSM for each participant,
describing the protocol from their point of view. This FSM is used to
automatically generate a Rust API, which uses the type system to check
conformance of an implementation to this FSM. \Cref{fig:rumpsteak_files} shows
concrete examples of each stage. \cref{fig:example_scribble} shows a Scribble
representation of a global type; \cref{fig:example_automata} displays one of the
FSMs that is projected from this Scribble file, this FSM is a simple DOT
graph~\cite{GraphVizDOT}; and finally, an FSM is used to generate a Rust API,
which we show an excerpt of in \cref{fig:example_rust}. These steps are further
detailed in the following paragraphs.

\paragraph{Projection} To guarantee safety in our double buffering example using
\mpst, we define a global type $\gt_\textsf{DB}$ for the protocol. This protocol
has three participants: a source \ppt{s}, a kernel \ppt{k} (which controls both
of the buffers) and a sink \ppt{t}. We show this global type below, and its
corresponding Scribble description in~\cref{fig:example_scribble}.
\begin{multline*}
  \gt_\textsf{DB} = \gtrec{x}\gtmsgs{k}{s}\mathit{ready}.\gtmsgs{s}{k} \\
  \mathit{value}.\gtmsgs{t}{k}\mathit{ready}.\gtmsgs{k}{t}\mathit{value}.\gtvar{x}\gtmsge\gtmsge\gtmsge\gtmsge
\end{multline*}
A global type is projected onto each participant to obtain a \emph{finite state
  machine} (FSM) $\efsm_i$ of its local interactions with other parties. For
instance, the kernel, whose projected type $\efsm_\ppt{k}$ is shown in
\cref{fig:example_automata},
\begin{enumerate*}[label=\textbf{(\arabic*)}, ref={\arabic*}]
  \item\label{itm:DoubleBufferingStart} informs the source that it is ready to
  receive;
  \item receives a value from the source;
  \item waits for the sink to become ready;
  \item sends a value to the sink; and
  \item repeats from step~\ref{itm:DoubleBufferingStart}.
\end{enumerate*}
In session type syntax~\cite{Yoshida2020}, $!$ and $?$ denote \emph{send} and
\emph{receive} respectively.

\begin{figure}
  \centering
  \begin{subfigure}{.6\linewidth}
    \centering
    \begin{tikzpicture}[>=to, -to, thick, font=\footnotesize, initial left, initial distance=1.5ex, initial text={}, state/.style={draw, circle, node distance=1cm and 1.6cm, inner sep=3pt}, every path/.style={every node/.style={fill=white}}]
      \node[state,initial] (1) {};
      \node[state] (2) [right=of 1] {};
      \node[state] (3) [right=of 2] {};
      \node[state] (4) [below=of 3] {};
      \node[state] (5) [left=of 4] {};

      \path (1) edge node {$\tout{s}\mathit{ready}$} (2);
      \path (2) edge node {$\tout{s}\mathit{ready}$} (3);
      \path (3) edge node {$\tin{s}\mathit{value}$} (4);
      \path (4) edge node {$\tin{t}\mathit{ready}$} (5);
      \path (5) edge node {$\tout{t}\mathit{value}$} (2);
    \end{tikzpicture}
    \caption{Optimised FSM for \(\ppt{k}\) ($\oefsm_\ppt{k}$)}
    \label{fig:DoubleBufferingOFSM}
  \end{subfigure}

  \begin{subfigure}{.5\linewidth}
    \centering
    \begin{tikzpicture}[>=to, -to, thick, font=\footnotesize, initial left, initial distance=1.5ex, initial text={}, state/.style={draw, circle, node distance=1cm and 1.6cm, inner sep=3pt}, every path/.style={every node/.style={fill=white}}]
      \node[state,initial] (1) {};
      \node[state] (2) [right=of 1] {};

      \path (1) edge[bend left] node {$\tout{k}\mathit{ready}$} (2);
      \path (2) edge[bend left] node {$\tin{k}\mathit{value}$} (1);
    \end{tikzpicture}
    \caption{Projected FSM for \(\ppt{t}\) (\(\efsm_\ppt{t}\))}
  \end{subfigure}\begin{subfigure}{.5\linewidth}
    \centering
    \begin{tikzpicture}[>=to, -to, thick, font=\footnotesize, initial left, initial distance=1.5ex, initial text={}, state/.style={draw, circle, node distance=1cm and 1.6cm, inner sep=3pt}, every path/.style={every node/.style={fill=white}}]
      \node[state,initial] (1) {};
      \node[state] (2) [right=of 1] {};

      \path (1) edge[bend left] node {$\tin{k}\mathit{ready}$} (2);
      \path (2) edge[bend left] node {$\tout{k}\mathit{value}$} (1);
    \end{tikzpicture}
    \caption{Projected FSM for \(\ppt{s}\) (\(\efsm_\ppt{s}\))}
  \end{subfigure}
  \caption{FSMs for roles \(\ppt{k}\), \(\ppt{t}\) and \(\ppt{s}\) of the double buffering protocol.}
\end{figure}
\paragraph{Asynchronous message reordering} Unfortunately, global types cannot
represent overlapping communication. Therefore, the projection $\efsm_\ppt{k}$
cannot achieve the simultaneous interactions we saw in
\cref{fig:DoubleBuffering}. In practice, developers use \amr to produce an
optimised FSM for the kernel $\oefsm_\ppt{k}$ (shown in
\cref{fig:DoubleBufferingOFSM}). Here, the kernel initially sends 2
$\mathit{ready}$ messages to the source. This allows the source to write to the
second buffer while the sink is busy reading from the first. Note that the
asynchronous queue is effectively acting as the second buffer---the second
message from the source waits in the queue while the kernel is processing the
first.

Crucially, \rumpsteak verifies that $\oefsm_\ppt{k}$ is safe to use in the place
of $\efsm_\ppt{k}$ without causing deadlocks or other communication errors.
Otherwise, we would be throwing away the safety benefits that come with \mpst.
To achieve this, we must determine that $\oefsm_\ppt{k}$ is an
\emph{asynchronous subtype} of $\efsm_\ppt{k}$, which we perform using our
algorithm presented in \cref{sec:Theory}.

\paragraph{API design} Once we arrive at an optimised FSM $\oefsm_i$ for each
participant, our challenge is to create a Rust API $\api_i$, which uses Rust's
type checker to ensure that a developer-written process $\proc_i$ conforms to
$\oefsm_i$ (a relevant introduction to the Rust programming language can be found in
Jung's thesis~\cite{Jung_2020}, Chapter~8). In the top-down approach, this API
is automatically generated from an optimised FSM.

To illustrate, we show the API for the kernel ($\api_\ppt{k}$) in
\cref{lst:API}, which checks conformance to $\oefsm_\ppt{k}$. To ensure that our
API remains readable by developers and to eliminate extensive boilerplate code,
we make use of Rust's procedural macros \cite{RustProceduralMacros}. By
decorating types with \code{\#[...]}, these macros perform additional
compile-time code generation.


\begin{description}
  \item[Roles (Participants).] Each role is represented as a struct, which
    stores its communication channels with other roles. The struct for the
    kernel (\cref{line:Role}) contains channels to and from \ppt{s} and \ppt{t}.
    Developers can in fact use any custom channel that implements Rust's
    standard \code{Sink} or \code{Stream} interfaces~\cite{Futures} for
    asynchronous sends and receives respectively. This approach minimises the
    expensive creation of channels in cases where only bounded or unidirectional
    channels are required.

    Our \code{\#[derive(Role)]} macro generates methods for programmatically
    retrieving these channels from the struct. Moreover, an optional
    \code{\#[derive(Roles)]} macro can be applied on a struct containing every
    role to also generate code for automatically instantiating all roles at
    once. This will create the necessary combination of channels and assign them
    to the correct structs in order to reduce human error.

  \item[Sessions.] Following the approach of
    \multicrusty~\cite{Lagaillardie2020}, we build a set of \emph{generic
      primitives} to construct a simple API. For instance, the \code{Send}
    primitive (\cref{line:SendPrimitive}) takes a role, label and continuation
    as generic parameters. In contrast to the standard approach of creating a
    type for every state \cite{Hu2016}, these primitives reduce the number of
    types required and avoid arbitrary naming of these `state types'. For
    brevity, our API elides two additional parameters used to store channels at
    runtime, which are reinserted with the \code{\#[session]} macro.

\begin{lstlisting}[language=Rust, label={lst:API}, caption={\rumpsteak API for the kernel.}, float=t]
#[derive(Role)]
#[message(Label)]
struct K(
  #[route(S)] Channel,
  #[route(T)] Channel
);@\label{line:Role}@

#[derive(Message)]
enum Label {@\label{line:Message}@
  Ready(Ready),
  Value(Value),
}

struct Ready;@\label{line:ReadyLabel}@
struct Value(i32);@\label{line:CopyLabel}@

#[session]
type Kernel = Send<S, Ready, KernelLoop>;

#[session]
struct KernelLoop(Send<S, Ready, Receive<S, Value,@\label{line:SendPrimitive}@
    Receive<T, Ready, Send<T, Value, Self>>>>);
\end{lstlisting}

  \item[Labels.] Internally, \rumpsteak sends a \code{Label} enum
    (\cref{line:Message}) over reusable channels to communicate with other
    participants. Each label is represented as a type
    (\crefrange{line:ReadyLabel}{line:CopyLabel}) and our
    \code{\#[derive(Message)]} macro generates methods for converting to and
    from the \code{Label} enum.

  \item[Choice.] The kernel's API does not contain choice but we show an example
    of this below. Choice is represented as an enum where each branch contains
    the label sent/received and a continuation. This design allows processes to
    pattern match on external choices to determine which label was received.
    Methods allowing the enum to be used with \code{Branch} (an \emph{external}
    choice, \cref{line:BranchPrimitive}) or \code{Select} (an \emph{internal}
    choice) are also generated with the \code{\#[session]} macro. Even so, the
    enum is still necessary since Rust's lack of variadic generics means choice
    cannot be easily implemented as its own primitive.
    \begin{lstlisting}[language=Rust]
#[session]
enum Choice {
  Continue(Continue, Branch<A, Self>),@\label{line:BranchPrimitive}@
  Stop(Stop, End),
}
    \end{lstlisting}
\end{description}

\paragraph{Process implementation} Using the API $\api_\ppt{k}$, the developer
writes an implementation for the process $\proc_\ppt{k}$; we show an example in
\cref{lst:Process}. We discuss how our API use Rust's type system to check that
$\proc_\ppt{k}$ conforms to the protocol.
\begin{lstlisting}[language=Rust, caption={Process implementation for the kernel.}, label={lst:Process}, float=t]
async fn kernel(role: &mut K) -> Result<()> {
  try_session(role, |s: Kernel<'_, _>| async {@\label{line:TrySession}@
    let mut t = s.send(Ready).await?;
    loop {@\label{line:LoopBottom}@
      let s = t.into_session().send(Ready).await?;
      let (Value(value), s) = s.receive().await?;
      let (Ready, s) = s.receive().await?;
      t = s.send(Value(value)).await?;
    }
  }).await
}
\end{lstlisting}
\begin{description}
  \item[Linearity.] The linear usage of channels is checked by Rust's
    \emph{affine type system}, preventing channels from being used multiple
    times. When a primitive is executed, it consumes itself, preventing reuse,
    and returns its continuation.

    Developers are prevented from constructing primitives directly using
    visibility modifiers. They must instead use \code{try\_session}
    (\cref{line:TrySession}). This function accepts a reference to the role
    being implemented and a closure (or function pointer) to its process
    implementation. The closure takes the input session type as an argument and
    returns the terminal type \code{End}. If a session is discarded, thereby
    breaking linearity, then the developer will have no \code{End} to return and
    Rust's compiler will complain that the closure does not satisfy its type.

  \item[Infinite recursion.] At first glance, it seems impossible to implement
    processes with infinitely recursive types using this approach. Nevertheless,
    for types without an \code{End} primitive, such as \code{Kernel}, we can use
    an infinite loop (\cref{line:LoopBottom}) to get around this problem.
    Conveniently, infinite loops are assigned \code{Infallible}, Rust's never
    (or bottom) type, which can be implicitly cast to any other type. This
    allows the type of the loop to be coerced to \code{End}, enabling the
    closure to pass the type checker as before.

  \item[Channel reuse.] We allow roles to be reused across sessions since the
    channels they contain are usually expensive to create. Crucially, to prevent
    communication mismatches between different sessions, we must ensure that the
    same role is not used in multiple sessions at once. Therefore,
    \code{try\_session} takes an \emph{exclusive} reference to the role, causing
    Rust's borrow checker to enforce this requirement.
\end{description}

\subsection{Bottom-Up Approach}
\label{subsec:bottomup}
In the top-down approach, we generate a Rust API $\api_i$ from an optimised FSM
$\oefsm_i$. In the bottom-up approach (\cref{fig:bottomup}), we do the reverse:
we \textbf{\emph{serialise}} each API $\api_i$ to obtain an FSM $\oefsm_i$.
Next, we use \kmc on the set of FSMs $\oefsm_{1 \ldots n}$. If they are indeed
compatible, then the processes $\proc_{1 \ldots n}$, which implement their
respective APIs, are free from deadlocks.

To perform the serialisation of an API to an FSM we provide a Rust function
\code{serialize<S>() -> Fsm} (this is a simplified version). It takes a session
type API (such as \code{Kernel} from \cref{sec:TopDown}) as a generic type
parameter \code{S} and returns its corresponding FSM. This FSM can be printed in
a variety of formats and passed into the \kmc tool for verification.

\subsection{Hybrid Approach}
\label{subsec:hybrid}
The bottom-up approach is convenient since code generation can be quite opaque
to the developer. However, using \kmc over asynchronous subtyping is not ideal
either---analysing the local types for all participants in the protocol at once
is challenging to do scalably (see \cref{sec:Evaluation}).

Therefore, we also propose a third, hybrid approach (\cref{fig:hybridapproach}).
In this workflow, a global type $\gt$ is provided by the developer and projected
to obtain the FSMs $\efsm_{1 \ldots n}$ as before. Rather than the developer
proposing the optimised FSMs $\oefsm_{1 \ldots n}$ directly, they instead
simply write the APIs $\api_{1 \ldots n}$ (as in the bottom-up approach). These
are serialised to $\oefsm_{1 \ldots n}$ which can (as in the top-down approach)
be checked for safety against $\efsm_{1 \ldots n}$ using asynchronous subtyping.


==> arxiv/sections/theory.tex <==
\section{A Sound Asynchronous Multiparty Session Subtyping Algorithm}
\label{sec:Theory}

This section proposes an algorithm for asynchronous multiparty subtyping
(\cref{sec:SoundAlgorithm}), shows its soundness (\cref{thm:Soundness}),
termination (\cref{thm:Termination}) and complexity (\cref{thm:Complexity}), and
sketches its implementation.

We begin by formally defining global and local session types. In the remainder
of this section, we will omit sorts $S$ from the syntax to simplify the
presentation.

\begin{definition}[Global and local types]
  \label{def:syntax}
  \[
    \begin{array}{rclr}
      S   & \bnfas & \code{i32} \bnfalt \code{u32} \bnfalt \code{i64} \bnfalt \code{u64} \bnfalt \ldots \\
      \gt & \bnfas & \gtend  \bnfalt  \gtmsg{p}{q}{\ell_i(S_i).\gt_i}_{i
        \in I}
      \bnfalt \gtrec{t}\gt
      \bnfalt  \gtvar{t}                                                                                \\
      \lt & \bnfas & \tend
      \bnfalt
      \tsel{i \in I} \tout{p}\ell_i(S_i).\lt_i
      \bnfalt  \tbra{i \in I} \tin{p}\ell_i(S_i).\lt_i
      \bnfalt  \trec{t}{\lt}
      \bnfalt  \tvar{t}
    \end{array}
  \]
  $\tsel{i \in I} \tout{p}\ell_i(S_i).\lt_i$ and $\tbra{i \in I}
    \tin{p}\ell_i(S_i).\lt_i$ represent \emph{internal} and \emph{external}
  choices respectively where $!$ and $?$ denote send and receive respectively,
  and all $\ell_i$ are pairwise distinct.
\end{definition}

Defining sound message reordering is non-trivial since it may introduce
deadlocks, as shown in the example below.

\begin{example}[Correct/incorrect \amr]
  \label{ex:amr}
  Consider the following local types
  \begin{center}
    \begin{tabular}{cc}
      \(\lt_Q = \tin{p}\ell_1.\tout{p}\ell_2.\tend\) &
      \(\lt_P = \tout{q}\ell_1.\tin{q}\ell_2.\tend\)
    \end{tabular}
  \end{center}
  which are given by projecting a global type\\
  \centerline{
    $\gtmsg{p}{q}{\ell_1.\gtmsg{q}{p}{\ell_2.\tend}}$.
  }

  Reordering the actions of \(\ppt{q}\) to become \(\lt_Q^\prime =
  \tout{p}\ell_2.\tin{p}\ell_1.\tend\), first sending before receiving
  the from, retains deadlock-freedom as messages are stored in queues and their
  reception can be delayed. However, if instead we reorder \(\ppt{p}\)'s to
  become \(\lt_P^\prime = \tin{q}\ell_2.\tout{q}\ell_1.\tend\), we
  arrive at a deadlock since both processes are simultaneously expecting to
  receive a message that has not yet been sent.
  %	\begin{center}
  %	\begin{tabular}{cc}
  %%		\(\lt_Q = \tin{p}\ell(S).\tout{p}\ell(S).\tend\) &
  %%		\(\lt_P = \tout{q}\ell(S).\tin{q}\ell(S).\tend\)\\
  %		\(\lt_Q^\prime = \tout{p}\ell(S).\tin{p}\ell(S).\tend\) &
  %		\(\lt_P^\prime = \tin{q}\ell(S).\tout{q}\ell(S).\tend\)
  %	\end{tabular}
  %	\end{center}
\end{example}


\subsection{Precise Asynchronous Multiparty Session Subtyping}
\label{sec:PreciseSubtyping}

\emph{Multiparty session subtyping} formulates \emph{refinement} for
communication protocols with more than two communicating processes. A process
implementing a session type $\lt$ can be safely used whenever a process
implementing one of its supertypes $\lt'$ is expected. This applies in any
context, ensuring that no deadlocks or other communication errors will be
introduced. Replacing the implementation of $\lt'$ with that of the subtype
$\lt$ may allow for more \emph{optimised} communication patterns as we have
seen. \citet{Ghilezan2021} present the \emph{precise} asynchronous subtyping
relation $\leq$ for multiparty session processes. Precision is characterised by
both \emph{soundness} (safe process replacement is guaranteed) and
\emph{completeness} (any extension of the relation is unsound).

Crucially, asynchronous subtyping supports the optimisation of communications.
Under certain conditions, the subtype can anticipate some input/output actions
occurring in the supertype, performing them \emph{earlier} than prescribed to
achieve the most flexible and precise subtyping. Such reorderings can take two
forms:
\begin{enumerate}[label=\textbf{R\arabic*.},ref=\textbf{R\arabic*}]
  \item\label{itm:ReorderA} anticipating an input from participant $\ppt{p}$
  before a finite number of inputs that are not from $\ppt{p}$; or
  \item\label{itm:ReorderB} anticipating an output to participant $\ppt{p}$
  before a finite number of inputs (from any participant), and also before other
  outputs that are not to $\ppt{p}$.
\end{enumerate}
To denote such reorderings, two kinds of finite sequences of inputs/outputs are
defined by \cite{Ghilezan2021}, where $\ppt{p} \neq \ppt{q}$. $\refa{p}$ is a
sequence containing receives from participants that are not $\ppt{p}$;
$\refb{p}$ is a sequence containing receives from \emph{any} participant
(\(\ppt{r} = \ppt{p}\) is allowed) as well as sends to
participants that are not $\ppt{p}$.
\begin{center}
  \small
  $\ \refa{p}\! ::= \!\tin{q}\ell \bnfalt \tin{q}\ell.\refa{p} \quad \refb{p} \! ::= \! \enskip \tin{r}\ell \bnfalt \tout{q}\ell \bnfalt \tin{r}\ell.\refb{p} \bnfalt \tout{q}\ell.\refb{p}$
\end{center}
The \emph{tree refinement relation} $\lesssim$ is defined coinductively on
infinite session type trees that contain only single-inputs (SI) and
single-outputs (SO). We leave the formal definition of $\lesssim$ in
\cite{Ghilezan2021} and shall explain its essence with our sound
algorithm. Based on $\lesssim$, the subtyping relation $\leq$ for all types
(including internal and external choice) is given as
\vspace{-4mm}
\begin{prooftree}
  \small
  \def\defaultHypSeparation{\hskip 2.5pt}
  \AxiomC{$\forall U \in \so{T}$}
  \AxiomC{$\forall V' \in \si{T'}$}
  \AxiomC{$\exists W \in \si{U}$}
  \AxiomC{$\exists W' \in \so{V'}$}
  \AxiomC{$W \lesssim W'$}
  \QuinaryInfC{$\lt \leq \lt'$}
\end{prooftree}
where $\so{T}$ (resp. $\si{T}$) is the minimal set of trees containing only
single \emph{outputs} (resp. \emph{inputs}) of the session type tree $T$. Using
existential quantifiers for $\si{U}$ and $\so{V'}$ allows external choices to be
added and internal choices to be removed (see \inApp{subsec:subtypeex} for
examples of $\leq$).

\subsection{Our Algorithm}
\label{sec:SoundAlgorithm}

The precise asynchronous subtyping in \cite{Ghilezan2021} is
\emph{undecidable}---even when limited to two participants, as proven
in~\cite{Lange2017}. This subsection introduces our \emph{practical} algorithm
which is \emph{sound} and \emph{terminates}, through the use of a bound on
recursion.

\paragraph{Prefixes} We first define reduction rules for finite single-input and
single-output (SISO) session type \emph{prefixes}.

\begin{definition}[Prefix reduction]
  \label{def:prefix}
  Let us define the syntax of \emph{prefixes} as
  \(
  \begin{array}{lclr}
    \pi, \rho  \bnfas   \epsilon
    \bnfalt  \tout{p}\ell(S)
    \bnfalt  \tin{p}\ell(S)
    \bnfalt  \pi_1.\pi_2
  \end{array}
  \)
  where ``$.$'' denotes the concatenation operator. We define the reduction
  $\pi \reduce \pi'$ as the smallest relation that ensures
  \begingroup
  \small
  \begin{equation*}
    \begin{array}{rrcl}
      \ruleRed{i}
                                                          & \pair{\tin{p}\ell.\pi}{\tin{p}\ell.\pi'}
                                                          & \reduce                                  & \pair{\pi}{\pi'}          \\
      \ruleRed{o}                                         &
      \pair{\tout{p}\ell.\pi}{\tout{p}\ell.\pi'}          & \reduce                                  &
      \pair{\pi}{\pi'}                                                                                                           \\
      \ruleRedA                                           &
      \pair{\tin{p}\ell.\pi}{\refa{p}.\tin{p}\ell.\pi'}   & \reduce                                  & \pair{\pi}{\refa{p}.\pi'} \\
      \ruleRedB                                           &
      \pair{\tout{p}\ell.\pi}{\refb{p}.\tout{p}\ell.\pi'} & \reduce                                  & \pair{\pi}{\refb{p}.\pi'}
    \end{array}
  \end{equation*}
  \endgroup
\end{definition}
\noindent\ruleRed{i} and \ruleRed{o} erase the top input and output prefixes
respectively; \ruleRedA{} formalises \ref{itm:ReorderA} from
\cref{sec:PreciseSubtyping} (permuting the input $\tin{p}\ell$) while
\ruleRedB{} represents \ref{itm:ReorderB} (permuting the output $\tout{p}\ell$).

\begin{example}[Prefix reduction]
\label{ex:prefix}
In \cref{ex:amr}, We can consider both \(\lt_Q\) and \(\lt_P\) as prefixes since
they already contain no choice. The (safe) reordering \(\lt_Q'\) can be achieved
using \ruleRedB, where $\refb{p} = \tin{p}\ell_1$: 
\begin{equation*}
	\begin{array}{rc}
		&\pair{\tout{p}\ell_2.\tin{p}\ell_1.\tend}{\tin{p}\ell_1.\tout{p}\ell_2.\tend}\\
		\ruleRedB{} & \pair{\tin{p}\ell_1.\tend}{\tin{p}\ell_1.\tend}
	\end{array}
\end{equation*}
\noindent On the other hand, the (unsafe)
reordering \(\lt_P'\) cannot be achieved with \ruleRedA, since $\refa{q} =
  \tout{q}\ell_1$ violates the definition of $\refa{q}$.
\end{example}

\begin{figure}[t]
  {\small
    \begin{prooftree}
      \RightLabel{\ruleAlg{init}}
      \AxiomC{$\epsilon; \nil \vdash_k \triple{\epsilon}{\lt}{n} \leq \triple{\epsilon}{\lt'}{n}$}
      \AxiomC{$k, n \in \mathbb{N}$}
      \BinaryInfC{$\lt \leq \lt'$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{}
      \RightLabel{\ruleAlg{end}}
      \UnaryInfC{$\rho; \Sigma \vdash_k \triple{\epsilon}{\tend}{n} \leq \triple{\epsilon}{\tend}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$\Sigma\map{\pair{\pi}{\lt} \leq \pair{\pi'}{\lt'}} = \rho\quad \act{\rho'} \supseteq \act{\pi'}$}
      \RightLabel{\ruleAlg{asm}}
      \UnaryInfC{$\rho.\rho'; \Sigma \vdash_k \triple{\pi}{\lt}{n} \leq \triple{\pi'}{\lt'}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$\pair{\pi_1}{\pi'_1} \reduce \pair{\pi_2}{\pi'_2}$}
      \AxiomC{$\rho; \Sigma \vdash_k \triple{\pi_2}{\lt}{n} \leq \triple{\pi'_2}{\lt'}{n'}$}
      \RightLabel{\ruleAlg{sub}}
      \BinaryInfC{$\rho; \Sigma \vdash_k \triple{\pi_1}{\lt}{n} \leq \triple{\pi'_1}{\lt'}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$\forall i \in I.\
          \forall j \in J.\
          \rho . \tout{p} \ell_i; \Sigma \vdash_k \triple{\pi . \tout{p} \ell_i}{\lt_i}{n} \leq \triple{\pi' . \tin{q} \ell_j}{\lt'_j}{n'}$}
      \RightLabel{\ruleAlg{oi}}
      \UnaryInfC{$\rho; \Sigma \vdash_k \triple{\pi}{\tsel{i \in I} \tout{p} \ell_i . \lt_i}{n} \leq \triple{\pi'}{\tbra{j \in J} \tin{q} \ell_j. \lt'_j}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$\forall i \in I.\
          \exists j \in J.\
          \rho . \tout{p} \ell_i; \Sigma \vdash_k \triple{\pi . \tout{p} \ell_i}{\lt_i}{n} \leq \triple{\pi' . \tout{q} \ell_j}{\lt'_j}{n'}$}
      \RightLabel{\ruleAlg{oo}}
      \UnaryInfC{$\rho; \Sigma \vdash_k \triple{\pi}{\tsel{i \in I} \tout{p} \ell_i. \lt_i}{n} \leq \triple{\pi'}{\tsel{j \in J} \tout{q} \ell_j. \lt'_j}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$\forall j \in J.\
          \exists i \in I.\
          \rho . \tin{p} \ell_i; \Sigma \vdash_k \triple{\pi . \tin{p} \ell_i}{\lt_i}{n} \leq \triple{\pi' . \tin{q} \ell_j}{\lt'_j}{n'}$}
      \RightLabel{\ruleAlg{ii}}
      \UnaryInfC{$\rho; \Sigma \vdash_k \triple{\pi}{\tbra{i \in I} \tin{p} \ell_i. \lt_i}{n} \leq \triple{\pi'}{\tbra{j \in J} \tin{q} \ell_j. \lt'_j}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$\exists i \in I.\
          \exists j \in J.\
          \rho . \tin{p} \ell_i; \Sigma \vdash_k \triple{\pi . \tin{p} \ell_i}{\lt_i}{n} \leq \triple{\pi' . \tout{q} \ell_j}{\lt'_j}{n'}$}
      \RightLabel{\ruleAlg{io}}
      \UnaryInfC{$\rho; \Sigma \vdash_k \triple{\pi}{\tbra{i \in I} \tin{p} \ell_i. \lt_i}{n} \leq \triple{\pi'}{\tsel{j \in J} \tout{q} \ell_j. \lt'_j}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$
          \begin{array}{c}
            \Sigma'=\Sigma\map{\pair{\pi}{\trec{t}{\lt}} \leq \pair{\pi'}{\lt'} \mapsto \rho} \\
            \rho; \Sigma' \vdash_k \triple{\pi}{\lt[\trec{t}{\lt} / \tvar{t}]}{n -
              1} \leq \triple{\pi'}{\lt'}{n'}
            \quad\quad n > 0
          \end{array}
        $}
      \RightLabel{\ruleAlg{\(\mu\)l}}
      \UnaryInfC{$\rho; \Sigma \vdash_k \triple{\pi}{\trec{t}{\lt}}{n} \leq \triple{\pi'}{\lt'}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$
          \begin{array}{c}
            \Sigma'=\Sigma\map{\pair{\pi}{\lt} \leq \pair{\pi'}{\trec{t}{\lt'}} \mapsto \rho} \\
            \rho; \Sigma' \vdash_k \triple{\pi}{\lt}{n} \leq
            \triple{\pi'}{\lt'[\trec{t}{\lt'} / \tvar{t}]}{n' - 1}\quad\quad n' > 0
          \end{array}$}
      \RightLabel{\ruleAlg{\(\mu\)r}}
      \UnaryInfC{$\rho; \Sigma \vdash_k \triple{\pi}{\lt}{n} \leq \triple{\pi'}{\trec{t}{\lt'}}{n'}$}
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{$
          \begin{array}{c}
            \rho; \Sigma \vdash_{k - 1} \triple{\pi}{\lt}{n} \leq \triple{\pi'}{\lt'}{n'} \\
            \rho; \Sigma \vdash_{k - 1} \triple{\pi'}{\lt'}{n'} \leq
            \triple{\pi''}{\lt''}{n''}
            \quad k > 0
          \end{array}
        $}
      \RightLabel{\ruleAlg{tra}}
      \UnaryInfC{$\rho; \Sigma \vdash_k \triple{\pi}{\lt}{n} \leq \triple{\pi''}{\lt''}{n''}$}
    \end{prooftree}
  }
  \caption{Asynchronous subtyping algorithm rules.}
  \label{fig:SubtypingAlgorithm}
  \vspace*{-0.5cm}
\end{figure}

\paragraph{Algorithm} We define the rules for our asynchronous subtyping
algorithm in \cref{fig:SubtypingAlgorithm}, following the style of
\cite{Gay2005}. Our rules use the function $\act{W}$, the set of input and
output actions of $\pi$ such that $\act{\epsilon} = \nil$,
$\act{\tin{p}\ell.\pi} = \{\tin{p}\} \cup \act{\pi}$ and $\act{\tout{p}\ell.\pi}
  = \{\tout{p}\} \cup \act{\pi}$.

Our algorithm operates on triples of $\triple{\pi}{\lt}{n}$, where $\pi$ is a
session prefix and $n$ is a bound on the number of recursions to unroll. We keep
track of $\rho$, a prefix containing all actions in the subtype seen so far, and
$\Sigma$, a set of subtyping assumptions. Each assumption in $\Sigma$ is
associated with the value of $\rho$ as it was at the time of the assumption. An
additional bound $k$ is included to limit applications of \ruleAlg{tra} rule. We
use our algorithm to check whether $\lt$ is a subtype of $\lt'$ by beginning
with the \ruleAlg{init} rule. If a proof derivation can be found then we
conclude that $\lt \leq \lt'$. If not, then either $\lt \not\leq \lt'$ or $\lt
  \leq \lt'$ but this cannot be shown by our algorithm since $\leq$ is undecidable
(hence our algorithm cannot be complete).

Our algorithm works as follows:
\begin{enumerate*}[label=\textbf{(\arabic*)}]
  \item\label{itm:AlgorithmStart} If both prefixes $\pi$ and $\pi'$ are empty
  and $\lt = \lt' = \tend$, then we have nothing left to check and we terminate
  with success (\ruleAlg{end}).
  \item If $\pair{\pi}{\lt} \leq \pair{\pi'}{\lt'}$ is already in our set of
  assumptions, then we perform a check on $\pi'$ to ensure that no actions have
  been forgotten by the subtype (see \inApp{sec:Proofs} for more detail). If this
  check passes, then we terminate with success (\ruleAlg{asm}).
  \item We attempt to reduce the pair of prefixes $\pair{\pi}{\pi'}$. If we can,
  then the algorithm repeats from \ref{itm:AlgorithmStart} (\ruleAlg{sub}).
  \item If not, we try to pop one action from the start of both $\lt$ and $\lt'$
  and push them to the end of $\pi$ and $\pi'$ respectively. If this is
  possible, we repeat from \ref{itm:AlgorithmStart} (\ruleAlg{oi,oo,ii,io}).
  Note that the quantifiers permit subtyping for internal and external choices.
  For example, \ruleAlg{oo} says $\lt$ is a subtype of $\lt'$ if it has a subset
  of $\lt'$'s internal choices (defined with $\forall i\in I . \exists j\in J$).
  \item Otherwise, we attempt to unroll recursion in $\lt$ (resp.~$\lt'$),
  decrement the bound $n$ (resp.~$n'$) by one and repeat from
  \ref{itm:AlgorithmStart}. If the bound is already zero, we instead terminate
  (\ruleAlg{\(\mu\)l,\(\mu\)r}).
\end{enumerate*}

\paragraph{Double buffering example} We show the execution of our algorithm to
check the optimised type from \cref{sec:Overview} for the kernel in the double
buffering protocol (i.e.\ $\lt \leq \lt'$).
\vspace{-5mm}
\begin{center}
  \small
  \begin{equation*}
    \lt = \tout{s}\mathit{ready}.\lt' \quad
    \lt' = \trec{x}{\tout{s}\mathit{ready}.\tin{s}\mathit{copy}.\tin{t}\mathit{ready}.\tout{t}\mathit{copy}.\tvar{x}}
  \end{equation*}
  \begin{prooftree}
    \AxiomC{\((\ast)\)}
    \AxiomC{$(\dagger)$}
    \AxiomC{$(\ddagger)$}
    \AxiomC{(\(\star\))}
    \AxiomC{(\(\div\))}
    \AxiomC{$\act{\pi_1.\pi_2.\pi_3.\pi_4} \supseteq \act{\epsilon}$}
    \RightLabel{\ruleAlg{asm}}
    \UnaryInfC{$\rho_5; \Sigma_3 \vdash \triple{\epsilon}{\lt^\prime}{1} \leq \triple{\epsilon}{\lt^{\prime\prime}}{0} $}
    \RightLabel{\ruleAlg{sub}}
    \BinaryInfC{$\rho_5; \Sigma_3 \vdash \triple{\pi_4}{\lt^\prime}{1} \leq \triple{\pi_4}{\lt^{\prime\prime}}{0} $}
    \RightLabel{\ruleAlg{sub}}
    \BinaryInfC{$\rho_5; \Sigma_3 \vdash \triple{\pi_3.\pi_4}{\lt^\prime}{1} \leq \triple{\pi_3.\pi_4}{\lt^{\prime\prime}}{0} $}
    \RightLabel{\ruleAlg{sub}}
    \BinaryInfC{$\rho_5; \Sigma_3 \vdash \triple{\pi_2.\pi_3.\pi_4}{\lt^\prime}{1} \leq \triple{\pi_2.\pi_3.\pi_4}{\lt^{\prime\prime}}{0} $}
    \RightLabel{\ruleAlg{sub}}
    \BinaryInfC{$\rho_5; \Sigma_3 \vdash \triple{\pi_1.\pi_2.\pi_3.\pi_4}{\lt^\prime}{1} \leq \triple{\pi_2.\pi_3.\pi_4.\pi_1}{\lt^{\prime\prime}}{0} $}
    \RightLabel{\ruleAlg{oo}}
    \UnaryInfC{$\rho_4; \Sigma_3 \vdash \triple{\pi_1.\pi_2.\pi_3}{\tout{t}\mathit{copy}.\lt^\prime}{1} \leq \triple{\pi_2.\pi_3.\pi_4}{\tout{s}\mathit{ready}.\lt^{\prime\prime}}{0} $}
    \RightLabel{\ruleAlg{\(\mu\)r}}
    \UnaryInfC{$\rho_4; \Sigma_2 \vdash \triple{\pi_1.\pi_2.\pi_3}{\tout{t}\mathit{copy}.\lt^\prime}{1} \leq \triple{\pi_2.\pi_3.\pi_4}{\lt^\prime}{1} $}
    \RightLabel{\ruleAlg{io}}
    \UnaryInfC{$\rho_3; \Sigma_2 \vdash \triple{\pi_1.\pi_2}{\tin{t}\mathit{ready}.\tout{t}\mathit{copy}.\lt^\prime}{1} \leq \triple{\pi_2.\pi_3}{\tout{t}\mathit{copy}.\lt^\prime}{1} $}
    \RightLabel{\ruleAlg{ii}}
    \UnaryInfC{$\rho_2; \Sigma_2 \vdash \triple{\pi_1}{\lt^{\prime\prime}}{1} \leq \triple{\pi_2}{\tin{t}\mathit{ready}.\tout{t}\mathit{copy}.\lt^\prime}{1} $}
    \RightLabel{\ruleAlg{oi}}
    \UnaryInfC{$\rho_1; \Sigma_2 \vdash \triple{\epsilon}{\tout{s}\mathit{ready}.\lt^{\prime\prime}}{1} \leq \triple{\epsilon}{\lt^{\prime\prime}}{1} $}
    \RightLabel{\ruleAlg{\(\mu\)l}}
    \UnaryInfC{$\rho_1; \Sigma_1 \vdash \triple{\epsilon}{\lt^\prime}{2} \leq \triple{\epsilon}{\lt^{\prime\prime}}{1} $}
    \RightLabel{\ruleAlg{sub}}
    \def\defaultHypSeparation{\hskip -35pt}
    \BinaryInfC{$\rho_1; \Sigma_1 \vdash \triple{\pi_1}{\lt^\prime}{2} \leq \triple{\pi_1}{\lt^{\prime\prime}}{1} $}
    \RightLabel{\ruleAlg{oo}}
    \UnaryInfC{$\epsilon; \Sigma_1 \vdash \triple{\epsilon}{\lt}{2} \leq \triple{\epsilon}{\tout{s}\mathit{ready}.\lt^{\prime\prime}}{1} $}
    \RightLabel{\ruleAlg{\(\mu\)r}}
    \UnaryInfC{$\epsilon; \nil \vdash \triple{\epsilon}{\lt}{2} \leq \triple{\epsilon}{\lt^\prime}{2}$}
    \RightLabel{\ruleAlg{init}}
    \UnaryInfC{$\lt \leq \lt'$}
  \end{prooftree}
  \begin{gather*}
    \lt^{\prime\prime} = \tin{s}\mathit{copy}.\tin{t}\mathit{ready}.\tout{t}\mathit{copy}.\lt^\prime \\
    \pi_1 = \tout{s}\mathit{ready} \quad
    \pi_2 = \tin{s}\mathit{copy} \quad
    \pi_3 = \tin{t}\mathit{ready} \quad
    \pi_4 = \tout{t}\mathit{copy} \\
    \rho_1 = \pi_1 \quad
    \rho_2 = \rho_1.\pi_1 \quad
    \rho_3 = \rho_2.\pi_2 \quad
    \rho_4 = \rho_3.\pi_3 \quad
    \rho_5 = \rho_4.\pi_4
  \end{gather*}
  \begin{gather*}
    \Sigma_1 = \map{\pair{\epsilon}{\lt} \leq \pair{\epsilon}{\lt^\prime}\mapsto \epsilon} \\
    \Sigma_2 = \Sigma_1\map{\pair{\epsilon}{\lt^\prime} \leq \pair{\epsilon}{\lt^{\prime\prime}}\mapsto \tout{s}\mathit{ready}} \\
    \Sigma_3 = \Sigma_2\map{\pair{\pi_1.\pi_2.\pi_3}{\tout{t}\mathit{copy}.\lt^\prime}\leq \pair{\pi_2.\pi_3.\pi_4}{\lt^\prime}\mapsto\rho_4}
  \end{gather*}
  \begin{gather*}
    (\dagger) = \pair{\pi_1.\pi_2.\pi_3.\pi_4}{\pi_2.\pi_3.\pi_4.\pi_1} \reduce \pair{\pi_2.\pi_3.\pi_4}{\pi_2.\pi_3.\pi_4} \; \ruleRedA \\
    (\ddagger) = \pair{\pi_2.\pi_3.\pi_4}{\pi_2.\pi_3.\pi_4} \reduce \pair{\pi_3.\pi_4}{\pi_3.\pi_4} \; \ruleRed{i} \\
    (\star) = \pair{\pi_3.\pi_4}{\pi_3.\pi_4} \reduce \pair{\pi_4}{\pi_4} \; \ruleRed{i} \\
    (\ast) = \pair{\pi_1}{\pi_1} \reduce \pair{\epsilon}{\epsilon} \; \ruleRed{o} \quad
    (\div) = \pair{\pi_4}{\pi_4} \reduce \pair{\epsilon}{\epsilon} \; \ruleRed{o}
  \end{gather*}
\end{center}
See also \inApp{subsec:algorthmex} for the ring and alternating bit protocols
which include internal and external choices.

\paragraph{Properties} We prove the correctness and complexity of our algorithm.
See \inApp{sec:AppendixSubtyping} for the proofs. We define the size of prefixes
as $\tsize{\epsilon} = 0$ and $\tsize{\tin{p}\ell.\pi} =
  \tsize{\tout{p}\ell.\pi} = 1 + \tsize{\pi}$.

\begin{lemma}
  \label{thm:PrefixesTermination}
  Given finite prefixes $\pi$ and $\pi'$, $\pair{\pi}{\pi'}$ can be reduced only
  a finite number of times.
\end{lemma}

\begin{theorem}[Termination]
  \label{thm:Termination}
  Our subtyping algorithm always eventually terminates.
\end{theorem}

\begin{theorem}[Soundness]
  \label{thm:Soundness}
  Our subtyping algorithm is sound.
\end{theorem}

\begin{lemma}
  \label{thm:PrefixesComplexity}
  Given finite prefixes $\pi$ and $\pi'$, the time complexity of reducing
  $\pair{\pi}{\pi'}$ is $\oh(\min(\tsize{\pi}, \tsize{\pi'}))$.
\end{lemma}

\begin{theorem}[Complexity]
  \label{thm:Complexity}
  Consider $\lt$ and $\lt'$ as (possibly infinite) trees $\tr{\lt}$ and
  $\tr{\lt'}$ with \emph{asymptotic branching factors} $b$ and $b'$
  respectively~\cite{Edelkamp1998,Korf1985}. Our algorithm has time complexity
  $\oh(n\min(b, b')^n)$ and space complexity $\oh(n\min(b, b'))$ in the worst
  case to determine if $\lt \leq \lt'$ with bound $n$.
\end{theorem}

\paragraph{Algorithm implementation}
\label{sec:AlgorithmImplementation}

In practice, we make some minor alterations to the algorithm when implementing
it in \rumpsteak. As outlined in \cref{sec:Overview}, \rumpsteak acts on FSMs
rather than local types so we modify our bound-checking accordingly. We also
represent prefixes as lazily-removable lists for greater memory
efficiency---this additionally allows a slightly simplified termination
condition in the case of \ruleAlg{asm}. Finally, we provide some opportunities
for the algorithm to ``short circuit'' in cases where we can tell early that a
subtype is not valid. See \inApp{subsec:impalg} for more details.


==> arxiv/title.tex <==
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{Deadlock-Free Asynchronous Message Reordering in Rust with Multiparty Session Types}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Zak Cutner}
%\email{zachary.cutner17@imperial.ac.uk}
\orcid{0000-0001-7180-4530}
\affiliation{%
    \institution{Imperial College London}
    \city{London}
    \country{UK}
}

\author{Nobuko Yoshida}
%\email{n.yoshida@imperial.ac.uk}
\orcid{0000-0002-3925-8557}
\affiliation{%
    \institution{Imperial College London}
    \city{London}
    \country{UK}
}

\author{Martin Vassor}
%\email{m.vassor@imperial.ac.uk}
\orcid{ 0000-0002-2057-0495 }
\affiliation{%
    \institution{Imperial College London}
    \city{London}
    \country{UK}
}

%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
% \renewcommand{\shortauthors}{Trovato and Tobin, et al.}


==> sections/case_study.tex <==
\section{Case Study: HTTP Cache}
\label{sec:CaseStudy}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle, white, fill=black, thick, inner sep=1.25pt, outer sep=0pt] (char) {\sffamily\tiny\bfseries#1};}\hspace{1pt}}

\begin{figure}
  \centering
  \sffamily\footnotesize
  \setlength{\twemojiDefaultHeight}{14pt}
  \begin{tikzpicture}[-to, thick, node distance=1.4cm and 2.8cm, every path/.style={shorten >=0.1cm, shorten <=0.1cm}]
    \node[align=center] (C) {\twemoji{technologist}\\\textit{Client}};
    \node[align=center] (P) [right=of C] {\twemoji{desktop computer}\\\textit{Proxy}};
    \node[align=center] (O) [right=of P] {\twemoji{earth_africa}\\\textit{Origin}};
    \node[align=center] (D1) [below=of C] {\twemoji{minidisc}\\\textit{Cache}};
    \node[align=center] (D2) [below=of P] {\twemoji{minidisc}\\\textit{Cache}};
    \node[align=center] (D3) [below=of O] {\twemoji{minidisc}\\\textit{Cache}};

    \path (C) edge node[fill=white] {\circled{0} Request} (P);
    \path[above, bend right=20] (P) edge node {\circled{7} Response} (C);

    \path (P) edge node[fill=white] {\circled{5} Request} (O);
    \path[above, bend right=20] (O) edge node {\circled{6} Response} (P);

    \path[sloped, above, bend right=15] (P) edge node {\circled{1} Lock} (D1);
    \path[sloped] (D1) edge node[fill=white] {\circled{2} Locked} (P);

    \path[sloped, below, bend right=10] (P) edge node {\circled{3} Load} (D2);
    \path[sloped, below, bend right=10] (D2) edge node {\circled{4} Entry} (P);

    \path[sloped] (P) edge node[fill=white] {\circled{8} Store/Remove\textsuperscript{$\star$}} (D3);
    \path[sloped, above, bend left=15] (P) edge node {\circled{9} Unlock} (D3);
  \end{tikzpicture}
  \caption{Interactions in the caching case study (optional interactions are marked with $\star$).}
  \label{fig:Caching}
\end{figure}

Caches are important for the performance of web applications. When a
\emph{client} (e.g.\ a browser) makes an HTTP request to an \emph{origin} (i.e.\
a web server), a \emph{proxy} can often fulfil the request by using a previous
response stored in a \emph{cache}. This reduces strain on the origin since fewer
expensive responses have to be sent and can improve latency if the cache is
physically located closer to the client (this is the concept behind content
delivery networks).

Since \emph{static} resources can change frequently, the HTTP protocol contains
several methods for validating that cache entries are not expired---we make use
of \emph{entity tags}~\cite{Fielding2014}. Here, the origin gives each version
of a resource a unique identifier, which is included in the response. The cache
stores this identifier with each entry. When a new request is made for the same
resource, this identifier is sent to the origin to inexpensively confirm that
the response has not expired.

We build a caching protocol using a microservices architecture shown in
\cref{fig:Caching}. Importantly, the client and origin's implementations are
unaware of the existence of the proxy.

\begin{enumerate*}[start=0, label={\hspace{2pt}\protect\circled{\scriptsize\arabic*}}]
  \item The client makes a request to the origin that is intercepted by the
  proxy.
  \item The proxy locks the entry for that request in the cache. This prevents
  simultaneous requests causing the same response to be returned from the origin
  multiple times.
  \item The cache confirms that the resource has been successfully locked.
  \item The proxy loads the previously-stored response (if any) in the cache.
  \item This entry is returned to the proxy.
  \item The client's request is forwarded to the origin, including the entity
  tag if it was in the cache.
  \item The origin responds to the request.
  \item This response if forwarded to the client. If the origin's response
  simply confirmed that the entity tag was still valid, then the proxy sends the
  cached version.
  \item If the cache entry is empty or its previous value had expired, the new
  response is stored. If the response cannot be cached (e.g.\ it contains no
  entity tag), then this step is skipped and any existing cache entry is removed
  as appropriate.
  \item The cache entry is unlocked so that future requests can be made.
\end{enumerate*}

\begin{lstlisting}[language=Scribble, caption={Scribble protocol for the caching case study.}, label={lst:CachingScribble}, float=h]
global protocol Caching(role Client, role Proxy,
    role Cache, role Origin) {
  Request from Client to Proxy;
  Lock from Proxy to Cache;
  Locked from Cache to Proxy;
  Load from Proxy to Cache;
  Entry from Cache to Proxy;
  Request from Proxy to Origin;
  Response from Origin to Proxy;
  Response from Proxy to Client;
  rec Loop {
    choice at Proxy {
      Store from Proxy to Cache;
      continue Loop;
    } or {
      Remove from Proxy to Cache;
      continue Loop;
    } or {
      Unlock from Proxy to Cache;
    }
  }
}
\end{lstlisting}

To demonstrate that \rumpsteak is applicable to larger use cases like this
caching example, we provide an implementation in \rumpsteak using the Scribble
protocol shown in \cref{lst:CachingScribble}. We use Redis~\cite{Redis}, a
well-known in-memory database, for the cache. Each entry is indexed using a
combination of the request method (i.e.\ GET, POST, etc.), the path (e.g.\
\code{/index.html}) and the values of selected headers.

Moreover, to show that \rumpsteak can be used in real-world Rust applications,
our implementation integrates many popular libraries from Rust's \async/\await
ecosystem---Tokio~\cite{Tokio} for spawning concurrent asynchronous tasks,
Hyper~\cite{Hyper} for interfacing with HTTP and Fred~\cite{Fred} for
communicating with Redis. We distribute our implementation as a command-line
tool which can be used in practice as an HTTP cache.

